When Deep Learning Meets Smart Contracts

Ethereum has become a widely used platform to enable secure, Blockchain-based financial and business transactions. However, many identified bugs and vulnerabilities in smart contracts have led to serious financial losses, which raises serious concerns about smart contract security. Thus, there is a significant need to better maintain smart contract code and ensure its high reliability. In this research: (1) Firstly, we propose an automated deep learning based approach to learn structural code embeddings of smart contracts in Solidity, which is useful for clone detection, bug detection and contract validation on smart contracts. We apply our approach to more than 22K solidity contracts collected from the Ethereum blockchain, results show that the clone ratio of solidity code is at around 90%, much higher than traditional software. We collect a list of 52 known buggy smart contracts belonging to 10 kinds of common vulnerabilities as our bug database. Our approach can identify more than 1000 clone related bugs based on our bug databases efficiently and accurately. (2) Secondly, according to developers' feedback, we have implemented the approach in a web-based tool, named SmartEmbed, to facilitate Solidity developers for using our approach. Our tool can assist Solidity developers to efficiently identify repetitive smart contracts in the existing Ethereum blockchain, as well as checking their contract against a known set of bugs, which can help to improve the users' confidence in the reliability of the contract. We optimize the implementations of SmartEmbed which is sufficient in supporting developers in real-time for practical uses. The Ethereum ecosystem as well as the individual Solidity developer can both benefit from our research.

==> fontawesomesymbols-generic.tex <==
\def\faGlass{\faicon{glass}}
\def\faMusic{\faicon{music}}
\def\faSearch{\faicon{search}}
\def\faEnvelopeO{\faicon{envelope-o}}
\def\faHeart{\faicon{heart}}
\def\faStar{\faicon{star}}
\def\faStarO{\faicon{star-o}}
\def\faUser{\faicon{user}}
\def\faFilm{\faicon{film}}
\def\faThLarge{\faicon{th-large}}
\def\faTh{\faicon{th}}
\def\faThList{\faicon{th-list}}
\def\faCheck{\faicon{check}}
\def\faTimes{\faicon{times}}
\def\faSearchPlus{\faicon{search-plus}}
\def\faSearchMinus{\faicon{search-minus}}
\def\faPowerOff{\faicon{power-off}}
\def\faSignal{\faicon{signal}}
\def\faCog{\faicon{cog}}
\def\faTrashO{\faicon{trash-o}}
\def\faHome{\faicon{home}}
\def\faFileO{\faicon{file-o}}
\def\faClockO{\faicon{clock-o}}
\def\faRoad{\faicon{road}}
\def\faDownload{\faicon{download}}
\def\faArrowCircleODown{\faicon{arrow-circle-o-down}}
\def\faArrowCircleOUp{\faicon{arrow-circle-o-up}}
\def\faInbox{\faicon{inbox}}
\def\faPlayCircleO{\faicon{play-circle-o}}
\def\faRepeat{\faicon{repeat}}
\def\faRefresh{\faicon{refresh}}
\def\faListAlt{\faicon{list-alt}}
\def\faLock{\faicon{lock}}
\def\faFlag{\faicon{flag}}
\def\faHeadphones{\faicon{headphones}}
\def\faVolumeOff{\faicon{volume-off}}
\def\faVolumeDown{\faicon{volume-down}}
\def\faVolumeUp{\faicon{volume-up}}
\def\faQrcode{\faicon{qrcode}}
\def\faBarcode{\faicon{barcode}}
\def\faTag{\faicon{tag}}
\def\faTags{\faicon{tags}}
\def\faBook{\faicon{book}}
\def\faBookmark{\faicon{bookmark}}
\def\faPrint{\faicon{print}}
\def\faCamera{\faicon{camera}}
\def\faFont{\faicon{font}}
\def\faBold{\faicon{bold}}
\def\faItalic{\faicon{italic}}
\def\faTextHeight{\faicon{text-height}}
\def\faTextWidth{\faicon{text-width}}
\def\faAlignLeft{\faicon{align-left}}
\def\faAlignCenter{\faicon{align-center}}
\def\faAlignRight{\faicon{align-right}}
\def\faAlignJustify{\faicon{align-justify}}
\def\faList{\faicon{list}}
\def\faOutdent{\faicon{outdent}}
\def\faIndent{\faicon{indent}}
\def\faVideoCamera{\faicon{video-camera}}
\def\faPictureO{\faicon{picture-o}}
\def\faPencil{\faicon{pencil}}
\def\faMapMarker{\faicon{map-marker}}
\def\faAdjust{\faicon{adjust}}
\def\faTint{\faicon{tint}}
\def\faPencilSquareO{\faicon{pencil-square-o}}
\def\faShareSquareO{\faicon{share-square-o}}
\def\faCheckSquareO{\faicon{check-square-o}}
\def\faArrows{\faicon{arrows}}
\def\faStepBackward{\faicon{step-backward}}
\def\faFastBackward{\faicon{fast-backward}}
\def\faBackward{\faicon{backward}}
\def\faPlay{\faicon{play}}
\def\faPause{\faicon{pause}}
\def\faStop{\faicon{stop}}
\def\faForward{\faicon{forward}}
\def\faFastForward{\faicon{fast-forward}}
\def\faStepForward{\faicon{step-forward}}
\def\faEject{\faicon{eject}}
\def\faChevronLeft{\faicon{chevron-left}}
\def\faChevronRight{\faicon{chevron-right}}
\def\faPlusCircle{\faicon{plus-circle}}
\def\faMinusCircle{\faicon{minus-circle}}
\def\faTimesCircle{\faicon{times-circle}}
\def\faCheckCircle{\faicon{check-circle}}
\def\faQuestionCircle{\faicon{question-circle}}
\def\faInfoCircle{\faicon{info-circle}}
\def\faCrosshairs{\faicon{crosshairs}}
\def\faTimesCircleO{\faicon{times-circle-o}}
\def\faCheckCircleO{\faicon{check-circle-o}}
\def\faBan{\faicon{ban}}
\def\faArrowLeft{\faicon{arrow-left}}
\def\faArrowRight{\faicon{arrow-right}}
\def\faArrowUp{\faicon{arrow-up}}
\def\faArrowDown{\faicon{arrow-down}}
\def\faShare{\faicon{share}}
\def\faExpand{\faicon{expand}}
\def\faCompress{\faicon{compress}}
\def\faPlus{\faicon{plus}}
\def\faMinus{\faicon{minus}}
\def\faAsterisk{\faicon{asterisk}}
\def\faExclamationCircle{\faicon{exclamation-circle}}
\def\faGift{\faicon{gift}}
\def\faLeaf{\faicon{leaf}}
\def\faFire{\faicon{fire}}
\def\faEye{\faicon{eye}}
\def\faEyeSlash{\faicon{eye-slash}}
\def\faExclamationTriangle{\faicon{exclamation-triangle}}
\def\faPlane{\faicon{plane}}
\def\faCalendar{\faicon{calendar}}
\def\faRandom{\faicon{random}}
\def\faComment{\faicon{comment}}
\def\faMagnet{\faicon{magnet}}
\def\faChevronUp{\faicon{chevron-up}}
\def\faChevronDown{\faicon{chevron-down}}
\def\faRetweet{\faicon{retweet}}
\def\faShoppingCart{\faicon{shopping-cart}}
\def\faFolder{\faicon{folder}}
\def\faFolderOpen{\faicon{folder-open}}
\def\faArrowsV{\faicon{arrows-v}}
\def\faArrowsH{\faicon{arrows-h}}
\def\faBarChart{\faicon{bar-chart}}
\def\faTwitterSquare{\faicon{twitter-square}}
\def\faFacebookSquare{\faicon{facebook-square}}
\def\faCameraRetro{\faicon{camera-retro}}
\def\faKey{\faicon{key}}
\def\faCogs{\faicon{cogs}}
\def\faComments{\faicon{comments}}
\def\faThumbsOUp{\faicon{thumbs-o-up}}
\def\faThumbsODown{\faicon{thumbs-o-down}}
\def\faStarHalf{\faicon{star-half}}
\def\faHeartO{\faicon{heart-o}}
\def\faSignOut{\faicon{sign-out}}
\def\faLinkedinSquare{\faicon{linkedin-square}}
\def\faThumbTack{\faicon{thumb-tack}}
\def\faExternalLink{\faicon{external-link}}
\def\faSignIn{\faicon{sign-in}}
\def\faTrophy{\faicon{trophy}}
\def\faGithubSquare{\faicon{github-square}}
\def\faUpload{\faicon{upload}}
\def\faLemonO{\faicon{lemon-o}}
\def\faPhone{\faicon{phone}}
\def\faSquareO{\faicon{square-o}}
\def\faBookmarkO{\faicon{bookmark-o}}
\def\faPhoneSquare{\faicon{phone-square}}
\def\faTwitter{\faicon{twitter}}
\def\faFacebook{\faicon{facebook}}
\def\faGithub{\faicon{github}}
\def\faUnlock{\faicon{unlock}}
\def\faCreditCard{\faicon{credit-card}}
\def\faRss{\faicon{rss}}
\def\faHddO{\faicon{hdd-o}}
\def\faBullhorn{\faicon{bullhorn}}
\def\faBell{\faicon{bell}}
\def\faCertificate{\faicon{certificate}}
\def\faHandORight{\faicon{hand-o-right}}
\def\faHandOLeft{\faicon{hand-o-left}}
\def\faHandOUp{\faicon{hand-o-up}}
\def\faHandODown{\faicon{hand-o-down}}
\def\faArrowCircleLeft{\faicon{arrow-circle-left}}
\def\faArrowCircleRight{\faicon{arrow-circle-right}}
\def\faArrowCircleUp{\faicon{arrow-circle-up}}
\def\faArrowCircleDown{\faicon{arrow-circle-down}}
\def\faGlobe{\faicon{globe}}
\def\faWrench{\faicon{wrench}}
\def\faTasks{\faicon{tasks}}
\def\faFilter{\faicon{filter}}
\def\faBriefcase{\faicon{briefcase}}
\def\faArrowsAlt{\faicon{arrows-alt}}
\def\faUsers{\faicon{users}}
\def\faLink{\faicon{link}}
\def\faCloud{\faicon{cloud}}
\def\faFlask{\faicon{flask}}
\def\faScissors{\faicon{scissors}}
\def\faFilesO{\faicon{files-o}}
\def\faPaperclip{\faicon{paperclip}}
\def\faFloppyO{\faicon{floppy-o}}
\def\faSquare{\faicon{square}}
\def\faBars{\faicon{bars}}
\def\faListUl{\faicon{list-ul}}
\def\faListOl{\faicon{list-ol}}
\def\faStrikethrough{\faicon{strikethrough}}
\def\faUnderline{\faicon{underline}}
\def\faTable{\faicon{table}}
\def\faMagic{\faicon{magic}}
\def\faTruck{\faicon{truck}}
\def\faPinterest{\faicon{pinterest}}
\def\faPinterestSquare{\faicon{pinterest-square}}
\def\faGooglePlusSquare{\faicon{google-plus-square}}
\def\faGooglePlus{\faicon{google-plus}}
\def\faMoney{\faicon{money}}
\def\faCaretDown{\faicon{caret-down}}
\def\faCaretUp{\faicon{caret-up}}
\def\faCaretLeft{\faicon{caret-left}}
\def\faCaretRight{\faicon{caret-right}}
\def\faColumns{\faicon{columns}}
\def\faSort{\faicon{sort}}
\def\faSortDesc{\faicon{sort-desc}}
\def\faSortAsc{\faicon{sort-asc}}
\def\faEnvelope{\faicon{envelope}}
\def\faLinkedin{\faicon{linkedin}}
\def\faUndo{\faicon{undo}}
\def\faGavel{\faicon{gavel}}
\def\faTachometer{\faicon{tachometer}}
\def\faCommentO{\faicon{comment-o}}
\def\faCommentsO{\faicon{comments-o}}
\def\faBolt{\faicon{bolt}}
\def\faSitemap{\faicon{sitemap}}
\def\faUmbrella{\faicon{umbrella}}
\def\faClipboard{\faicon{clipboard}}
\def\faLightbulbO{\faicon{lightbulb-o}}
\def\faExchange{\faicon{exchange}}
\def\faCloudDownload{\faicon{cloud-download}}
\def\faCloudUpload{\faicon{cloud-upload}}
\def\faUserMd{\faicon{user-md}}
\def\faStethoscope{\faicon{stethoscope}}
\def\faSuitcase{\faicon{suitcase}}
\def\faBellO{\faicon{bell-o}}
\def\faCoffee{\faicon{coffee}}
\def\faCutlery{\faicon{cutlery}}
\def\faFileTextO{\faicon{file-text-o}}
\def\faBuildingO{\faicon{building-o}}
\def\faHospitalO{\faicon{hospital-o}}
\def\faAmbulance{\faicon{ambulance}}
\def\faMedkit{\faicon{medkit}}
\def\faFighterJet{\faicon{fighter-jet}}
\def\faBeer{\faicon{beer}}
\def\faHSquare{\faicon{h-square}}
\def\faPlusSquare{\faicon{plus-square}}
\def\faAngleDoubleLeft{\faicon{angle-double-left}}
\def\faAngleDoubleRight{\faicon{angle-double-right}}
\def\faAngleDoubleUp{\faicon{angle-double-up}}
\def\faAngleDoubleDown{\faicon{angle-double-down}}
\def\faAngleLeft{\faicon{angle-left}}
\def\faAngleRight{\faicon{angle-right}}
\def\faAngleUp{\faicon{angle-up}}
\def\faAngleDown{\faicon{angle-down}}
\def\faDesktop{\faicon{desktop}}
\def\faLaptop{\faicon{laptop}}
\def\faTablet{\faicon{tablet}}
\def\faMobile{\faicon{mobile}}
\def\faCircleO{\faicon{circle-o}}
\def\faQuoteLeft{\faicon{quote-left}}
\def\faQuoteRight{\faicon{quote-right}}
\def\faSpinner{\faicon{spinner}}
\def\faCircle{\faicon{circle}}
\def\faReply{\faicon{reply}}
\def\faGithubAlt{\faicon{github-alt}}
\def\faFolderO{\faicon{folder-o}}
\def\faFolderOpenO{\faicon{folder-open-o}}
\def\faSmileO{\faicon{smile-o}}
\def\faFrownO{\faicon{frown-o}}
\def\faMehO{\faicon{meh-o}}
\def\faGamepad{\faicon{gamepad}}
\def\faKeyboardO{\faicon{keyboard-o}}
\def\faFlagO{\faicon{flag-o}}
\def\faFlagCheckered{\faicon{flag-checkered}}
\def\faTerminal{\faicon{terminal}}
\def\faCode{\faicon{code}}
\def\faReplyAll{\faicon{reply-all}}
\def\faStarHalfO{\faicon{star-half-o}}
\def\faLocationArrow{\faicon{location-arrow}}
\def\faCrop{\faicon{crop}}
\def\faCodeFork{\faicon{code-fork}}
\def\faChainBroken{\faicon{chain-broken}}
\def\faQuestion{\faicon{question}}
\def\faInfo{\faicon{info}}
\def\faExclamation{\faicon{exclamation}}
\def\faSuperscript{\faicon{superscript}}
\def\faSubscript{\faicon{subscript}}
\def\faEraser{\faicon{eraser}}
\def\faPuzzlePiece{\faicon{puzzle-piece}}
\def\faMicrophone{\faicon{microphone}}
\def\faMicrophoneSlash{\faicon{microphone-slash}}
\def\faShield{\faicon{shield}}
\def\faCalendarO{\faicon{calendar-o}}
\def\faFireExtinguisher{\faicon{fire-extinguisher}}
\def\faRocket{\faicon{rocket}}
\def\faMaxcdn{\faicon{maxcdn}}
\def\faChevronCircleLeft{\faicon{chevron-circle-left}}
\def\faChevronCircleRight{\faicon{chevron-circle-right}}
\def\faChevronCircleUp{\faicon{chevron-circle-up}}
\def\faChevronCircleDown{\faicon{chevron-circle-down}}
\def\faHtml5{\faicon{html5}}
\def\faCss3{\faicon{css3}}
\def\faAnchor{\faicon{anchor}}
\def\faUnlockAlt{\faicon{unlock-alt}}
\def\faBullseye{\faicon{bullseye}}
\def\faEllipsisH{\faicon{ellipsis-h}}
\def\faEllipsisV{\faicon{ellipsis-v}}
\def\faRssSquare{\faicon{rss-square}}
\def\faPlayCircle{\faicon{play-circle}}
\def\faTicket{\faicon{ticket}}
\def\faMinusSquare{\faicon{minus-square}}
\def\faMinusSquareO{\faicon{minus-square-o}}
\def\faLevelUp{\faicon{level-up}}
\def\faLevelDown{\faicon{level-down}}
\def\faCheckSquare{\faicon{check-square}}
\def\faPencilSquare{\faicon{pencil-square}}
\def\faExternalLinkSquare{\faicon{external-link-square}}
\def\faShareSquare{\faicon{share-square}}
\def\faCompass{\faicon{compass}}
\def\faCaretSquareODown{\faicon{caret-square-o-down}}
\def\faCaretSquareOUp{\faicon{caret-square-o-up}}
\def\faCaretSquareORight{\faicon{caret-square-o-right}}
\def\faEur{\faicon{eur}}
\def\faGbp{\faicon{gbp}}
\def\faUsd{\faicon{usd}}
\def\faInr{\faicon{inr}}
\def\faJpy{\faicon{jpy}}
\def\faRub{\faicon{rub}}
\def\faKrw{\faicon{krw}}
\def\faBtc{\faicon{btc}}
\def\faFile{\faicon{file}}
\def\faFileText{\faicon{file-text}}
\def\faSortAlphaAsc{\faicon{sort-alpha-asc}}
\def\faSortAlphaDesc{\faicon{sort-alpha-desc}}
\def\faSortAmountAsc{\faicon{sort-amount-asc}}
\def\faSortAmountDesc{\faicon{sort-amount-desc}}
\def\faSortNumericAsc{\faicon{sort-numeric-asc}}
\def\faSortNumericDesc{\faicon{sort-numeric-desc}}
\def\faThumbsUp{\faicon{thumbs-up}}
\def\faThumbsDown{\faicon{thumbs-down}}
\def\faYoutubeSquare{\faicon{youtube-square}}
\def\faYoutube{\faicon{youtube}}
\def\faXing{\faicon{xing}}
\def\faXingSquare{\faicon{xing-square}}
\def\faYoutubePlay{\faicon{youtube-play}}
\def\faDropbox{\faicon{dropbox}}
\def\faStackOverflow{\faicon{stack-overflow}}
\def\faInstagram{\faicon{instagram}}
\def\faFlickr{\faicon{flickr}}
\def\faAdn{\faicon{adn}}
\def\faBitbucket{\faicon{bitbucket}}
\def\faBitbucketSquare{\faicon{bitbucket-square}}
\def\faTumblr{\faicon{tumblr}}
\def\faTumblrSquare{\faicon{tumblr-square}}
\def\faLongArrowDown{\faicon{long-arrow-down}}
\def\faLongArrowUp{\faicon{long-arrow-up}}
\def\faLongArrowLeft{\faicon{long-arrow-left}}
\def\faLongArrowRight{\faicon{long-arrow-right}}
\def\faApple{\faicon{apple}}
\def\faWindows{\faicon{windows}}
\def\faAndroid{\faicon{android}}
\def\faLinux{\faicon{linux}}
\def\faDribbble{\faicon{dribbble}}
\def\faSkype{\faicon{skype}}
\def\faFoursquare{\faicon{foursquare}}
\def\faTrello{\faicon{trello}}
\def\faFemale{\faicon{female}}
\def\faMale{\faicon{male}}
\def\faGratipay{\faicon{gratipay}}
\def\faSunO{\faicon{sun-o}}
\def\faMoonO{\faicon{moon-o}}
\def\faArchive{\faicon{archive}}
\def\faBug{\faicon{bug}}
\def\faVk{\faicon{vk}}
\def\faWeibo{\faicon{weibo}}
\def\faRenren{\faicon{renren}}
\def\faPagelines{\faicon{pagelines}}
\def\faStackExchange{\faicon{stack-exchange}}
\def\faArrowCircleORight{\faicon{arrow-circle-o-right}}
\def\faArrowCircleOLeft{\faicon{arrow-circle-o-left}}
\def\faCaretSquareOLeft{\faicon{caret-square-o-left}}
\def\faDotCircleO{\faicon{dot-circle-o}}
\def\faWheelchair{\faicon{wheelchair}}
\def\faVimeoSquare{\faicon{vimeo-square}}
\def\faTry{\faicon{try}}
\def\faPlusSquareO{\faicon{plus-square-o}}
\def\faSpaceShuttle{\faicon{space-shuttle}}
\def\faSlack{\faicon{slack}}
\def\faEnvelopeSquare{\faicon{envelope-square}}
\def\faWordpress{\faicon{wordpress}}
\def\faOpenid{\faicon{openid}}
\def\faUniversity{\faicon{university}}
\def\faGraduationCap{\faicon{graduation-cap}}
\def\faYahoo{\faicon{yahoo}}
\def\faGoogle{\faicon{google}}
\def\faReddit{\faicon{reddit}}
\def\faRedditSquare{\faicon{reddit-square}}
\def\faStumbleuponCircle{\faicon{stumbleupon-circle}}
\def\faStumbleupon{\faicon{stumbleupon}}
\def\faDelicious{\faicon{delicious}}
\def\faDigg{\faicon{digg}}
\def\faPiedPiperPp{\faicon{pied-piper-pp}}
\def\faPiedPiperAlt{\faicon{pied-piper-alt}}
\def\faDrupal{\faicon{drupal}}
\def\faJoomla{\faicon{joomla}}
\def\faLanguage{\faicon{language}}
\def\faFax{\faicon{fax}}
\def\faBuilding{\faicon{building}}
\def\faChild{\faicon{child}}
\def\faPaw{\faicon{paw}}
\def\faSpoon{\faicon{spoon}}
\def\faCube{\faicon{cube}}
\def\faCubes{\faicon{cubes}}
\def\faBehance{\faicon{behance}}
\def\faBehanceSquare{\faicon{behance-square}}
\def\faSteam{\faicon{steam}}
\def\faSteamSquare{\faicon{steam-square}}
\def\faRecycle{\faicon{recycle}}
\def\faCar{\faicon{car}}
\def\faTaxi{\faicon{taxi}}
\def\faTree{\faicon{tree}}
\def\faSpotify{\faicon{spotify}}
\def\faDeviantart{\faicon{deviantart}}
\def\faSoundcloud{\faicon{soundcloud}}
\def\faDatabase{\faicon{database}}
\def\faFilePdfO{\faicon{file-pdf-o}}
\def\faFileWordO{\faicon{file-word-o}}
\def\faFileExcelO{\faicon{file-excel-o}}
\def\faFilePowerpointO{\faicon{file-powerpoint-o}}
\def\faFileImageO{\faicon{file-image-o}}
\def\faFileArchiveO{\faicon{file-archive-o}}
\def\faFileAudioO{\faicon{file-audio-o}}
\def\faFileVideoO{\faicon{file-video-o}}
\def\faFileCodeO{\faicon{file-code-o}}
\def\faVine{\faicon{vine}}
\def\faCodepen{\faicon{codepen}}
\def\faJsfiddle{\faicon{jsfiddle}}
\def\faLifeRing{\faicon{life-ring}}
\def\faCircleONotch{\faicon{circle-o-notch}}
\def\faRebel{\faicon{rebel}}
\def\faEmpire{\faicon{empire}}
\def\faGitSquare{\faicon{git-square}}
\def\faGit{\faicon{git}}
\def\faHackerNews{\faicon{hacker-news}}
\def\faTencentWeibo{\faicon{tencent-weibo}}
\def\faQq{\faicon{qq}}
\def\faWeixin{\faicon{weixin}}
\def\faPaperPlane{\faicon{paper-plane}}
\def\faPaperPlaneO{\faicon{paper-plane-o}}
\def\faHistory{\faicon{history}}
\def\faCircleThin{\faicon{circle-thin}}
\def\faHeader{\faicon{header}}
\def\faParagraph{\faicon{paragraph}}
\def\faSliders{\faicon{sliders}}
\def\faShareAlt{\faicon{share-alt}}
\def\faShareAltSquare{\faicon{share-alt-square}}
\def\faBomb{\faicon{bomb}}
\def\faFutbolO{\faicon{futbol-o}}
\def\faTty{\faicon{tty}}
\def\faBinoculars{\faicon{binoculars}}
\def\faPlug{\faicon{plug}}
\def\faSlideshare{\faicon{slideshare}}
\def\faTwitch{\faicon{twitch}}
\def\faYelp{\faicon{yelp}}
\def\faNewspaperO{\faicon{newspaper-o}}
\def\faWifi{\faicon{wifi}}
\def\faCalculator{\faicon{calculator}}
\def\faPaypal{\faicon{paypal}}
\def\faGoogleWallet{\faicon{google-wallet}}
\def\faCcVisa{\faicon{cc-visa}}
\def\faCcMastercard{\faicon{cc-mastercard}}
\def\faCcDiscover{\faicon{cc-discover}}
\def\faCcAmex{\faicon{cc-amex}}
\def\faCcPaypal{\faicon{cc-paypal}}
\def\faCcStripe{\faicon{cc-stripe}}
\def\faBellSlash{\faicon{bell-slash}}
\def\faBellSlashO{\faicon{bell-slash-o}}
\def\faTrash{\faicon{trash}}
\def\faCopyright{\faicon{copyright}}
\def\faAt{\faicon{at}}
\def\faEyedropper{\faicon{eyedropper}}
\def\faPaintBrush{\faicon{paint-brush}}
\def\faBirthdayCake{\faicon{birthday-cake}}
\def\faAreaChart{\faicon{area-chart}}
\def\faPieChart{\faicon{pie-chart}}
\def\faLineChart{\faicon{line-chart}}
\def\faLastfm{\faicon{lastfm}}
\def\faLastfmSquare{\faicon{lastfm-square}}
\def\faToggleOff{\faicon{toggle-off}}
\def\faToggleOn{\faicon{toggle-on}}
\def\faBicycle{\faicon{bicycle}}
\def\faBus{\faicon{bus}}
\def\faIoxhost{\faicon{ioxhost}}
\def\faAngellist{\faicon{angellist}}
\def\faCc{\faicon{cc}}
\def\faIls{\faicon{ils}}
\def\faMeanpath{\faicon{meanpath}}
\def\faBuysellads{\faicon{buysellads}}
\def\faConnectdevelop{\faicon{connectdevelop}}
\def\faDashcube{\faicon{dashcube}}
\def\faForumbee{\faicon{forumbee}}
\def\faLeanpub{\faicon{leanpub}}
\def\faSellsy{\faicon{sellsy}}
\def\faShirtsinbulk{\faicon{shirtsinbulk}}
\def\faSimplybuilt{\faicon{simplybuilt}}
\def\faSkyatlas{\faicon{skyatlas}}
\def\faCartPlus{\faicon{cart-plus}}
\def\faCartArrowDown{\faicon{cart-arrow-down}}
\def\faDiamond{\faicon{diamond}}
\def\faShip{\faicon{ship}}
\def\faUserSecret{\faicon{user-secret}}
\def\faMotorcycle{\faicon{motorcycle}}
\def\faStreetView{\faicon{street-view}}
\def\faHeartbeat{\faicon{heartbeat}}
\def\faVenus{\faicon{venus}}
\def\faMars{\faicon{mars}}
\def\faMercury{\faicon{mercury}}
\def\faTransgender{\faicon{transgender}}
\def\faTransgenderAlt{\faicon{transgender-alt}}
\def\faVenusDouble{\faicon{venus-double}}
\def\faMarsDouble{\faicon{mars-double}}
\def\faVenusMars{\faicon{venus-mars}}
\def\faMarsStroke{\faicon{mars-stroke}}
\def\faMarsStrokeV{\faicon{mars-stroke-v}}
\def\faMarsStrokeH{\faicon{mars-stroke-h}}
\def\faNeuter{\faicon{neuter}}
\def\faGenderless{\faicon{genderless}}
\def\faFacebookOfficial{\faicon{facebook-official}}
\def\faPinterestP{\faicon{pinterest-p}}
\def\faWhatsapp{\faicon{whatsapp}}
\def\faServer{\faicon{server}}
\def\faUserPlus{\faicon{user-plus}}
\def\faUserTimes{\faicon{user-times}}
\def\faBed{\faicon{bed}}
\def\faViacoin{\faicon{viacoin}}
\def\faTrain{\faicon{train}}
\def\faSubway{\faicon{subway}}
\def\faMedium{\faicon{medium}}
\def\faYCombinator{\faicon{y-combinator}}
\def\faOptinMonster{\faicon{optin-monster}}
\def\faOpencart{\faicon{opencart}}
\def\faExpeditedssl{\faicon{expeditedssl}}
\def\faBatteryFull{\faicon{battery-full}}
\def\faBatteryThreeQuarters{\faicon{battery-three-quarters}}
\def\faBatteryHalf{\faicon{battery-half}}
\def\faBatteryQuarter{\faicon{battery-quarter}}
\def\faBatteryEmpty{\faicon{battery-empty}}
\def\faMousePointer{\faicon{mouse-pointer}}
\def\faICursor{\faicon{i-cursor}}
\def\faObjectGroup{\faicon{object-group}}
\def\faObjectUngroup{\faicon{object-ungroup}}
\def\faStickyNote{\faicon{sticky-note}}
\def\faStickyNoteO{\faicon{sticky-note-o}}
\def\faCcJcb{\faicon{cc-jcb}}
\def\faCcDinersClub{\faicon{cc-diners-club}}
\def\faClone{\faicon{clone}}
\def\faBalanceScale{\faicon{balance-scale}}
\def\faHourglassO{\faicon{hourglass-o}}
\def\faHourglassStart{\faicon{hourglass-start}}
\def\faHourglassHalf{\faicon{hourglass-half}}
\def\faHourglassEnd{\faicon{hourglass-end}}
\def\faHourglass{\faicon{hourglass}}
\def\faHandRockO{\faicon{hand-rock-o}}
\def\faHandPaperO{\faicon{hand-paper-o}}
\def\faHandScissorsO{\faicon{hand-scissors-o}}
\def\faHandLizardO{\faicon{hand-lizard-o}}
\def\faHandSpockO{\faicon{hand-spock-o}}
\def\faHandPointerO{\faicon{hand-pointer-o}}
\def\faHandPeaceO{\faicon{hand-peace-o}}
\def\faTrademark{\faicon{trademark}}
\def\faRegistered{\faicon{registered}}
\def\faCreativeCommons{\faicon{creative-commons}}
\def\faGg{\faicon{gg}}
\def\faGgCircle{\faicon{gg-circle}}
\def\faTripadvisor{\faicon{tripadvisor}}
\def\faOdnoklassniki{\faicon{odnoklassniki}}
\def\faOdnoklassnikiSquare{\faicon{odnoklassniki-square}}
\def\faGetPocket{\faicon{get-pocket}}
\def\faWikipediaW{\faicon{wikipedia-w}}
\def\faSafari{\faicon{safari}}
\def\faChrome{\faicon{chrome}}
\def\faFirefox{\faicon{firefox}}
\def\faOpera{\faicon{opera}}
\def\faInternetExplorer{\faicon{internet-explorer}}
\def\faTelevision{\faicon{television}}
\def\faContao{\faicon{contao}}
\def\fa500Px{\faicon{500px}}
\def\faAmazon{\faicon{amazon}}
\def\faCalendarPlusO{\faicon{calendar-plus-o}}
\def\faCalendarMinusO{\faicon{calendar-minus-o}}
\def\faCalendarTimesO{\faicon{calendar-times-o}}
\def\faCalendarCheckO{\faicon{calendar-check-o}}
\def\faIndustry{\faicon{industry}}
\def\faMapPin{\faicon{map-pin}}
\def\faMapSigns{\faicon{map-signs}}
\def\faMapO{\faicon{map-o}}
\def\faMap{\faicon{map}}
\def\faCommenting{\faicon{commenting}}
\def\faCommentingO{\faicon{commenting-o}}
\def\faHouzz{\faicon{houzz}}
\def\faVimeo{\faicon{vimeo}}
\def\faBlackTie{\faicon{black-tie}}
\def\faFonticons{\faicon{fonticons}}
\def\faRedditAlien{\faicon{reddit-alien}}
\def\faEdge{\faicon{edge}}
\def\faCreditCardAlt{\faicon{credit-card-alt}}
\def\faCodiepie{\faicon{codiepie}}
\def\faModx{\faicon{modx}}
\def\faFortAwesome{\faicon{fort-awesome}}
\def\faUsb{\faicon{usb}}
\def\faProductHunt{\faicon{product-hunt}}
\def\faMixcloud{\faicon{mixcloud}}
\def\faScribd{\faicon{scribd}}
\def\faPauseCircle{\faicon{pause-circle}}
\def\faPauseCircleO{\faicon{pause-circle-o}}
\def\faStopCircle{\faicon{stop-circle}}
\def\faStopCircleO{\faicon{stop-circle-o}}
\def\faShoppingBag{\faicon{shopping-bag}}
\def\faShoppingBasket{\faicon{shopping-basket}}
\def\faHashtag{\faicon{hashtag}}
\def\faBluetooth{\faicon{bluetooth}}
\def\faBluetoothB{\faicon{bluetooth-b}}
\def\faPercent{\faicon{percent}}
\def\faGitlab{\faicon{gitlab}}
\def\faWpbeginner{\faicon{wpbeginner}}
\def\faWpforms{\faicon{wpforms}}
\def\faEnvira{\faicon{envira}}
\def\faUniversalAccess{\faicon{universal-access}}
\def\faWheelchairAlt{\faicon{wheelchair-alt}}
\def\faQuestionCircleO{\faicon{question-circle-o}}
\def\faBlind{\faicon{blind}}
\def\faAudioDescription{\faicon{audio-description}}
\def\faVolumeControlPhone{\faicon{volume-control-phone}}
\def\faBraille{\faicon{braille}}
\def\faAssistiveListeningSystems{\faicon{assistive-listening-systems}}
\def\faAmericanSignLanguageInterpreting{\faicon{american-sign-language-interpreting}}
\def\faDeaf{\faicon{deaf}}
\def\faGlide{\faicon{glide}}
\def\faGlideG{\faicon{glide-g}}
\def\faSignLanguage{\faicon{sign-language}}
\def\faLowVision{\faicon{low-vision}}
\def\faViadeo{\faicon{viadeo}}
\def\faViadeoSquare{\faicon{viadeo-square}}
\def\faSnapchat{\faicon{snapchat}}
\def\faSnapchatGhost{\faicon{snapchat-ghost}}
\def\faSnapchatSquare{\faicon{snapchat-square}}
\def\faPiedPiper{\faicon{pied-piper}}
\def\faFirstOrder{\faicon{first-order}}
\def\faYoast{\faicon{yoast}}
\def\faThemeisle{\faicon{themeisle}}
\def\faGooglePlusOfficial{\faicon{google-plus-official}}
\def\faFontAwesome{\faicon{font-awesome}}
% aliases
\def\faCny{\faicon{cny}}\expandafter\def\csname faicon@cny\endcsname{\faicon{jpy}}
\def\faYCombinatorSquare{\faicon{y-combinator-square}}\expandafter\def\csname faicon@y-combinator-square\endcsname{\faicon{hacker-news}}
\def\faCab{\faicon{cab}}\expandafter\def\csname faicon@cab\endcsname{\faicon{taxi}}
\def\faToggleUp{\faicon{toggle-up}}\expandafter\def\csname faicon@toggle-up\endcsname{\faicon{caret-square-o-up}}
\def\faLifeBuoy{\faicon{life-buoy}}\expandafter\def\csname faicon@life-buoy\endcsname{\faicon{life-ring}}
\def\faFileZipO{\faicon{file-zip-o}}\expandafter\def\csname faicon@file-zip-o\endcsname{\faicon{file-archive-o}}
\def\faBitcoin{\faicon{bitcoin}}\expandafter\def\csname faicon@bitcoin\endcsname{\faicon{btc}}
\def\faAutomobile{\faicon{automobile}}\expandafter\def\csname faicon@automobile\endcsname{\faicon{car}}
\def\faPaste{\faicon{paste}}\expandafter\def\csname faicon@paste\endcsname{\faicon{clipboard}}
\def\faResistance{\faicon{resistance}}\expandafter\def\csname faicon@resistance\endcsname{\faicon{rebel}}
\def\faCopy{\faicon{copy}}\expandafter\def\csname faicon@copy\endcsname{\faicon{files-o}}
\def\faIntersex{\faicon{intersex}}\expandafter\def\csname faicon@intersex\endcsname{\faicon{transgender}}
\def\faHardOfHearing{\faicon{hard-of-hearing}}\expandafter\def\csname faicon@hard-of-hearing\endcsname{\faicon{deaf}}
\def\faMailReply{\faicon{mail-reply}}\expandafter\def\csname faicon@mail-reply\endcsname{\faicon{reply}}
\def\faSortDown{\faicon{sort-down}}\expandafter\def\csname faicon@sort-down\endcsname{\faicon{sort-desc}}
\def\faGe{\faicon{ge}}\expandafter\def\csname faicon@ge\endcsname{\faicon{empire}}
\def\faBattery2{\faicon{battery-2}}\expandafter\def\csname faicon@battery-2\endcsname{\faicon{battery-half}}
\def\faHandStopO{\faicon{hand-stop-o}}\expandafter\def\csname faicon@hand-stop-o\endcsname{\faicon{hand-paper-o}}
\def\faGroup{\faicon{group}}\expandafter\def\csname faicon@group\endcsname{\faicon{users}}
\def\faRotateRight{\faicon{rotate-right}}\expandafter\def\csname faicon@rotate-right\endcsname{\faicon{repeat}}
\def\faWon{\faicon{won}}\expandafter\def\csname faicon@won\endcsname{\faicon{krw}}
\def\faFa{\faicon{fa}}\expandafter\def\csname faicon@fa\endcsname{\faicon{font-awesome}}
\def\faHourglass3{\faicon{hourglass-3}}\expandafter\def\csname faicon@hourglass-3\endcsname{\faicon{hourglass-end}}
\def\faStarHalfEmpty{\faicon{star-half-empty}}\expandafter\def\csname faicon@star-half-empty\endcsname{\faicon{star-half-o}}
\def\faCut{\faicon{cut}}\expandafter\def\csname faicon@cut\endcsname{\faicon{scissors}}
\def\faToggleDown{\faicon{toggle-down}}\expandafter\def\csname faicon@toggle-down\endcsname{\faicon{caret-square-o-down}}
\def\faGooglePlusCircle{\faicon{google-plus-circle}}\expandafter\def\csname faicon@google-plus-circle\endcsname{\faicon{google-plus-official}}
\def\faSheqel{\faicon{sheqel}}\expandafter\def\csname faicon@sheqel\endcsname{\faicon{ils}}
\def\faDashboard{\faicon{dashboard}}\expandafter\def\csname faicon@dashboard\endcsname{\faicon{tachometer}}
\def\faSend{\faicon{send}}\expandafter\def\csname faicon@send\endcsname{\faicon{paper-plane}}
\def\faYc{\faicon{yc}}\expandafter\def\csname faicon@yc\endcsname{\faicon{y-combinator}}
\def\faToggleLeft{\faicon{toggle-left}}\expandafter\def\csname faicon@toggle-left\endcsname{\faicon{caret-square-o-left}}
\def\faWarning{\faicon{warning}}\expandafter\def\csname faicon@warning\endcsname{\faicon{exclamation-triangle}}
\def\faImage{\faicon{image}}\expandafter\def\csname faicon@image\endcsname{\faicon{picture-o}}
\def\faInstitution{\faicon{institution}}\expandafter\def\csname faicon@institution\endcsname{\faicon{university}}
\def\faFileMovieO{\faicon{file-movie-o}}\expandafter\def\csname faicon@file-movie-o\endcsname{\faicon{file-video-o}}
\def\faPhoto{\faicon{photo}}\expandafter\def\csname faicon@photo\endcsname{\faicon{picture-o}}
\def\faFileSoundO{\faicon{file-sound-o}}\expandafter\def\csname faicon@file-sound-o\endcsname{\faicon{file-audio-o}}
\def\faMortarBoard{\faicon{mortar-board}}\expandafter\def\csname faicon@mortar-board\endcsname{\faicon{graduation-cap}}
\def\faGittip{\faicon{gittip}}\expandafter\def\csname faicon@gittip\endcsname{\faicon{gratipay}}
\def\faHourglass2{\faicon{hourglass-2}}\expandafter\def\csname faicon@hourglass-2\endcsname{\faicon{hourglass-half}}
\def\faSupport{\faicon{support}}\expandafter\def\csname faicon@support\endcsname{\faicon{life-ring}}
\def\faEdit{\faicon{edit}}\expandafter\def\csname faicon@edit\endcsname{\faicon{pencil-square-o}}
\def\faHotel{\faicon{hotel}}\expandafter\def\csname faicon@hotel\endcsname{\faicon{bed}}
\def\faSoccerBallO{\faicon{soccer-ball-o}}\expandafter\def\csname faicon@soccer-ball-o\endcsname{\faicon{futbol-o}}
\def\faFilePictureO{\faicon{file-picture-o}}\expandafter\def\csname faicon@file-picture-o\endcsname{\faicon{file-image-o}}
\def\faClose{\faicon{close}}\expandafter\def\csname faicon@close\endcsname{\faicon{times}}
\def\faYcSquare{\faicon{yc-square}}\expandafter\def\csname faicon@yc-square\endcsname{\faicon{hacker-news}}
\def\faShekel{\faicon{shekel}}\expandafter\def\csname faicon@shekel\endcsname{\faicon{ils}}
\def\faDollar{\faicon{dollar}}\expandafter\def\csname faicon@dollar\endcsname{\faicon{usd}}
\def\faUnsorted{\faicon{unsorted}}\expandafter\def\csname faicon@unsorted\endcsname{\faicon{sort}}
\def\faReorder{\faicon{reorder}}\expandafter\def\csname faicon@reorder\endcsname{\faicon{bars}}
\def\faBattery3{\faicon{battery-3}}\expandafter\def\csname faicon@battery-3\endcsname{\faicon{battery-three-quarters}}
\def\faRupee{\faicon{rupee}}\expandafter\def\csname faicon@rupee\endcsname{\faicon{inr}}
\def\faRouble{\faicon{rouble}}\expandafter\def\csname faicon@rouble\endcsname{\faicon{rub}}
\def\faHourglass1{\faicon{hourglass-1}}\expandafter\def\csname faicon@hourglass-1\endcsname{\faicon{hourglass-start}}
\def\faAslInterpreting{\faicon{asl-interpreting}}\expandafter\def\csname faicon@asl-interpreting\endcsname{\faicon{american-sign-language-interpreting}}
\def\faTv{\faicon{tv}}\expandafter\def\csname faicon@tv\endcsname{\faicon{television}}
\def\faSave{\faicon{save}}\expandafter\def\csname faicon@save\endcsname{\faicon{floppy-o}}
\def\faToggleRight{\faicon{toggle-right}}\expandafter\def\csname faicon@toggle-right\endcsname{\faicon{caret-square-o-right}}
\def\faDedent{\faicon{dedent}}\expandafter\def\csname faicon@dedent\endcsname{\faicon{outdent}}
\def\faGear{\faicon{gear}}\expandafter\def\csname faicon@gear\endcsname{\faicon{cog}}
\def\faLegal{\faicon{legal}}\expandafter\def\csname faicon@legal\endcsname{\faicon{gavel}}
\def\faWechat{\faicon{wechat}}\expandafter\def\csname faicon@wechat\endcsname{\faicon{weixin}}
\def\faFacebookF{\faicon{facebook-f}}\expandafter\def\csname faicon@facebook-f\endcsname{\faicon{facebook}}
\def\faFeed{\faicon{feed}}\expandafter\def\csname faicon@feed\endcsname{\faicon{rss}}
\def\faBank{\faicon{bank}}\expandafter\def\csname faicon@bank\endcsname{\faicon{university}}
\def\faTurkishLira{\faicon{turkish-lira}}\expandafter\def\csname faicon@turkish-lira\endcsname{\faicon{try}}
\def\faUnlink{\faicon{unlink}}\expandafter\def\csname faicon@unlink\endcsname{\faicon{chain-broken}}
\def\faChain{\faicon{chain}}\expandafter\def\csname faicon@chain\endcsname{\faicon{link}}
\def\faGears{\faicon{gears}}\expandafter\def\csname faicon@gears\endcsname{\faicon{cogs}}
\def\faRmb{\faicon{rmb}}\expandafter\def\csname faicon@rmb\endcsname{\faicon{jpy}}
\def\faBattery1{\faicon{battery-1}}\expandafter\def\csname faicon@battery-1\endcsname{\faicon{battery-quarter}}
\def\faLifeBouy{\faicon{life-bouy}}\expandafter\def\csname faicon@life-bouy\endcsname{\faicon{life-ring}}
\def\faYen{\faicon{yen}}\expandafter\def\csname faicon@yen\endcsname{\faicon{jpy}}
\def\faBattery4{\faicon{battery-4}}\expandafter\def\csname faicon@battery-4\endcsname{\faicon{battery-full}}
\def\faBattery0{\faicon{battery-0}}\expandafter\def\csname faicon@battery-0\endcsname{\faicon{battery-empty}}
\def\faHandGrabO{\faicon{hand-grab-o}}\expandafter\def\csname faicon@hand-grab-o\endcsname{\faicon{hand-rock-o}}
\def\faMailReplyAll{\faicon{mail-reply-all}}\expandafter\def\csname faicon@mail-reply-all\endcsname{\faicon{reply-all}}
\def\faMobilePhone{\faicon{mobile-phone}}\expandafter\def\csname faicon@mobile-phone\endcsname{\faicon{mobile}}
\def\faRotateLeft{\faicon{rotate-left}}\expandafter\def\csname faicon@rotate-left\endcsname{\faicon{undo}}
\def\faEuro{\faicon{euro}}\expandafter\def\csname faicon@euro\endcsname{\faicon{eur}}
\def\faRuble{\faicon{ruble}}\expandafter\def\csname faicon@ruble\endcsname{\faicon{rub}}
\def\faRa{\faicon{ra}}\expandafter\def\csname faicon@ra\endcsname{\faicon{rebel}}
\def\faStarHalfFull{\faicon{star-half-full}}\expandafter\def\csname faicon@star-half-full\endcsname{\faicon{star-half-o}}
\def\faSortUp{\faicon{sort-up}}\expandafter\def\csname faicon@sort-up\endcsname{\faicon{sort-asc}}
\def\faMailForward{\faicon{mail-forward}}\expandafter\def\csname faicon@mail-forward\endcsname{\faicon{share}}
\def\faSigning{\faicon{signing}}\expandafter\def\csname faicon@signing\endcsname{\faicon{sign-language}}
\def\faFlash{\faicon{flash}}\expandafter\def\csname faicon@flash\endcsname{\faicon{bolt}}
\def\faLifeSaver{\faicon{life-saver}}\expandafter\def\csname faicon@life-saver\endcsname{\faicon{life-ring}}
\def\faFilePhotoO{\faicon{file-photo-o}}\expandafter\def\csname faicon@file-photo-o\endcsname{\faicon{file-image-o}}
\def\faDeafness{\faicon{deafness}}\expandafter\def\csname faicon@deafness\endcsname{\faicon{deaf}}
\def\faBarChartO{\faicon{bar-chart-o}}\expandafter\def\csname faicon@bar-chart-o\endcsname{\faicon{bar-chart}}
\def\faSendO{\faicon{send-o}}\expandafter\def\csname faicon@send-o\endcsname{\faicon{paper-plane-o}}
\def\faNavicon{\faicon{navicon}}\expandafter\def\csname faicon@navicon\endcsname{\faicon{bars}}
\def\faRemove{\faicon{remove}}\expandafter\def\csname faicon@remove\endcsname{\faicon{times}}


==> fontawesomesymbols-pdftex.tex <==
%% start of file `fontawesomesymbols-pdftex.tex'.
\expandafter\def\csname faicon@info\endcsname{{\FAone\symbol{0}}}
\expandafter\def\csname faicon@eraser\endcsname{{\FAone\symbol{1}}}
\expandafter\def\csname faicon@rss-square\endcsname{{\FAone\symbol{2}}}
\expandafter\def\csname faicon@external-link-square\endcsname{{\FAone\symbol{3}}}
\expandafter\def\csname faicon@caret-square-o-right\endcsname{{\FAone\symbol{4}}}
\expandafter\def\csname faicon@sort-alpha-desc\endcsname{{\FAone\symbol{5}}}
\expandafter\def\csname faicon@thumbs-up\endcsname{{\FAone\symbol{6}}}
\expandafter\def\csname faicon@thumbs-down\endcsname{{\FAone\symbol{7}}}
\expandafter\def\csname faicon@moon-o\endcsname{{\FAone\symbol{8}}}
\expandafter\def\csname faicon@pagelines\endcsname{{\FAone\symbol{9}}}
\expandafter\def\csname faicon@arrow-circle-o-right\endcsname{{\FAone\symbol{10}}}
\expandafter\def\csname faicon@caret-square-o-left\endcsname{{\FAone\symbol{11}}}
\expandafter\def\csname faicon@wheelchair\endcsname{{\FAone\symbol{12}}}
\expandafter\def\csname faicon@try\endcsname{{\FAone\symbol{13}}}
\expandafter\def\csname faicon@space-shuttle\endcsname{{\FAone\symbol{14}}}
\expandafter\def\csname faicon@slack\endcsname{{\FAone\symbol{15}}}
\expandafter\def\csname faicon@envelope-square\endcsname{{\FAone\symbol{16}}}
\expandafter\def\csname faicon@wordpress\endcsname{{\FAone\symbol{17}}}
\expandafter\def\csname faicon@openid\endcsname{{\FAone\symbol{18}}}
\expandafter\def\csname faicon@university\endcsname{{\FAone\symbol{19}}}
\expandafter\def\csname faicon@graduation-cap\endcsname{{\FAone\symbol{20}}}
\expandafter\def\csname faicon@yahoo\endcsname{{\FAone\symbol{21}}}
\expandafter\def\csname faicon@reddit-square\endcsname{{\FAone\symbol{22}}}
\expandafter\def\csname faicon@stumbleupon-circle\endcsname{{\FAone\symbol{23}}}
\expandafter\def\csname faicon@delicious\endcsname{{\FAone\symbol{24}}}
\expandafter\def\csname faicon@digg\endcsname{{\FAone\symbol{25}}}
\expandafter\def\csname faicon@pied-piper-pp\endcsname{{\FAone\symbol{26}}}
\expandafter\def\csname faicon@pied-piper-alt\endcsname{{\FAone\symbol{27}}}
\expandafter\def\csname faicon@drupal\endcsname{{\FAone\symbol{28}}}
\expandafter\def\csname faicon@joomla\endcsname{{\FAone\symbol{29}}}
\expandafter\def\csname faicon@fax\endcsname{{\FAone\symbol{30}}}
\expandafter\def\csname faicon@building\endcsname{{\FAone\symbol{31}}}
\expandafter\def\csname faicon@child\endcsname{{\FAone\symbol{32}}}
\expandafter\def\csname faicon@spoon\endcsname{{\FAone\symbol{33}}}
\expandafter\def\csname faicon@cube\endcsname{{\FAone\symbol{34}}}
\expandafter\def\csname faicon@cubes\endcsname{{\FAone\symbol{35}}}
\expandafter\def\csname faicon@behance\endcsname{{\FAone\symbol{36}}}
\expandafter\def\csname faicon@behance-square\endcsname{{\FAone\symbol{37}}}
\expandafter\def\csname faicon@steam\endcsname{{\FAone\symbol{38}}}
\expandafter\def\csname faicon@steam-square\endcsname{{\FAone\symbol{39}}}
\expandafter\def\csname faicon@recycle\endcsname{{\FAone\symbol{40}}}
\expandafter\def\csname faicon@car\endcsname{{\FAone\symbol{41}}}
\expandafter\def\csname faicon@taxi\endcsname{{\FAone\symbol{42}}}
\expandafter\def\csname faicon@tree\endcsname{{\FAone\symbol{43}}}
\expandafter\def\csname faicon@spotify\endcsname{{\FAone\symbol{44}}}
\expandafter\def\csname faicon@deviantart\endcsname{{\FAone\symbol{45}}}
\expandafter\def\csname faicon@soundcloud\endcsname{{\FAone\symbol{46}}}
\expandafter\def\csname faicon@file-word-o\endcsname{{\FAone\symbol{47}}}
\expandafter\def\csname faicon@file-excel-o\endcsname{{\FAone\symbol{48}}}
\expandafter\def\csname faicon@file-powerpoint-o\endcsname{{\FAone\symbol{49}}}
\expandafter\def\csname faicon@file-image-o\endcsname{{\FAone\symbol{50}}}
\expandafter\def\csname faicon@file-archive-o\endcsname{{\FAone\symbol{51}}}
\expandafter\def\csname faicon@file-audio-o\endcsname{{\FAone\symbol{52}}}
\expandafter\def\csname faicon@file-video-o\endcsname{{\FAone\symbol{53}}}
\expandafter\def\csname faicon@file-code-o\endcsname{{\FAone\symbol{54}}}
\expandafter\def\csname faicon@vine\endcsname{{\FAone\symbol{55}}}
\expandafter\def\csname faicon@codepen\endcsname{{\FAone\symbol{56}}}
\expandafter\def\csname faicon@jsfiddle\endcsname{{\FAone\symbol{57}}}
\expandafter\def\csname faicon@life-ring\endcsname{{\FAone\symbol{58}}}
\expandafter\def\csname faicon@circle-o-notch\endcsname{{\FAone\symbol{59}}}
\expandafter\def\csname faicon@git\endcsname{{\FAone\symbol{60}}}
\expandafter\def\csname faicon@hacker-news\endcsname{{\FAone\symbol{61}}}
\expandafter\def\csname faicon@paper-plane\endcsname{{\FAone\symbol{62}}}
\expandafter\def\csname faicon@paper-plane-o\endcsname{{\FAone\symbol{63}}}
\expandafter\def\csname faicon@history\endcsname{{\FAone\symbol{64}}}
\expandafter\def\csname faicon@circle-thin\endcsname{{\FAone\symbol{65}}}
\expandafter\def\csname faicon@header\endcsname{{\FAone\symbol{66}}}
\expandafter\def\csname faicon@paragraph\endcsname{{\FAone\symbol{67}}}
\expandafter\def\csname faicon@sliders\endcsname{{\FAone\symbol{68}}}
\expandafter\def\csname faicon@share-alt-square\endcsname{{\FAone\symbol{69}}}
\expandafter\def\csname faicon@bomb\endcsname{{\FAone\symbol{70}}}
\expandafter\def\csname faicon@futbol-o\endcsname{{\FAone\symbol{71}}}
\expandafter\def\csname faicon@tty\endcsname{{\FAone\symbol{72}}}
\expandafter\def\csname faicon@binoculars\endcsname{{\FAone\symbol{73}}}
\expandafter\def\csname faicon@plug\endcsname{{\FAone\symbol{74}}}
\expandafter\def\csname faicon@slideshare\endcsname{{\FAone\symbol{75}}}
\expandafter\def\csname faicon@twitch\endcsname{{\FAone\symbol{76}}}
\expandafter\def\csname faicon@yelp\endcsname{{\FAone\symbol{77}}}
\expandafter\def\csname faicon@newspaper-o\endcsname{{\FAone\symbol{78}}}
\expandafter\def\csname faicon@wifi\endcsname{{\FAone\symbol{79}}}
\expandafter\def\csname faicon@calculator\endcsname{{\FAone\symbol{80}}}
\expandafter\def\csname faicon@paypal\endcsname{{\FAone\symbol{81}}}
\expandafter\def\csname faicon@google-wallet\endcsname{{\FAone\symbol{82}}}
\expandafter\def\csname faicon@cc-mastercard\endcsname{{\FAone\symbol{83}}}
\expandafter\def\csname faicon@cc-discover\endcsname{{\FAone\symbol{84}}}
\expandafter\def\csname faicon@cc-paypal\endcsname{{\FAone\symbol{85}}}
\expandafter\def\csname faicon@cc-stripe\endcsname{{\FAone\symbol{86}}}
\expandafter\def\csname faicon@bell-slash\endcsname{{\FAone\symbol{87}}}
\expandafter\def\csname faicon@bell-slash-o\endcsname{{\FAone\symbol{88}}}
\expandafter\def\csname faicon@trash\endcsname{{\FAone\symbol{89}}}
\expandafter\def\csname faicon@copyright\endcsname{{\FAone\symbol{90}}}
\expandafter\def\csname faicon@at\endcsname{{\FAone\symbol{91}}}
\expandafter\def\csname faicon@eyedropper\endcsname{{\FAone\symbol{92}}}
\expandafter\def\csname faicon@birthday-cake\endcsname{{\FAone\symbol{93}}}
\expandafter\def\csname faicon@area-chart\endcsname{{\FAone\symbol{94}}}
\expandafter\def\csname faicon@pie-chart\endcsname{{\FAone\symbol{95}}}
\expandafter\def\csname faicon@line-chart\endcsname{{\FAone\symbol{96}}}
\expandafter\def\csname faicon@lastfm\endcsname{{\FAone\symbol{97}}}
\expandafter\def\csname faicon@lastfm-square\endcsname{{\FAone\symbol{98}}}
\expandafter\def\csname faicon@toggle-off\endcsname{{\FAone\symbol{99}}}
\expandafter\def\csname faicon@toggle-on\endcsname{{\FAone\symbol{100}}}
\expandafter\def\csname faicon@bicycle\endcsname{{\FAone\symbol{101}}}
\expandafter\def\csname faicon@bus\endcsname{{\FAone\symbol{102}}}
\expandafter\def\csname faicon@ioxhost\endcsname{{\FAone\symbol{103}}}
\expandafter\def\csname faicon@angellist\endcsname{{\FAone\symbol{104}}}
\expandafter\def\csname faicon@cc\endcsname{{\FAone\symbol{105}}}
\expandafter\def\csname faicon@ils\endcsname{{\FAone\symbol{106}}}
\expandafter\def\csname faicon@meanpath\endcsname{{\FAone\symbol{107}}}
\expandafter\def\csname faicon@buysellads\endcsname{{\FAone\symbol{108}}}
\expandafter\def\csname faicon@connectdevelop\endcsname{{\FAone\symbol{109}}}
\expandafter\def\csname faicon@forumbee\endcsname{{\FAone\symbol{110}}}
\expandafter\def\csname faicon@sellsy\endcsname{{\FAone\symbol{111}}}
\expandafter\def\csname faicon@shirtsinbulk\endcsname{{\FAone\symbol{112}}}
\expandafter\def\csname faicon@simplybuilt\endcsname{{\FAone\symbol{113}}}
\expandafter\def\csname faicon@skyatlas\endcsname{{\FAone\symbol{114}}}
\expandafter\def\csname faicon@cart-plus\endcsname{{\FAone\symbol{115}}}
\expandafter\def\csname faicon@cart-arrow-down\endcsname{{\FAone\symbol{116}}}
\expandafter\def\csname faicon@diamond\endcsname{{\FAone\symbol{117}}}
\expandafter\def\csname faicon@ship\endcsname{{\FAone\symbol{118}}}
\expandafter\def\csname faicon@user-secret\endcsname{{\FAone\symbol{119}}}
\expandafter\def\csname faicon@motorcycle\endcsname{{\FAone\symbol{120}}}
\expandafter\def\csname faicon@street-view\endcsname{{\FAone\symbol{121}}}
\expandafter\def\csname faicon@heartbeat\endcsname{{\FAone\symbol{122}}}
\expandafter\def\csname faicon@mars\endcsname{{\FAone\symbol{123}}}
\expandafter\def\csname faicon@mercury\endcsname{{\FAone\symbol{124}}}
\expandafter\def\csname faicon@transgender\endcsname{{\FAone\symbol{125}}}
\expandafter\def\csname faicon@transgender-alt\endcsname{{\FAone\symbol{126}}}
\expandafter\def\csname faicon@venus-double\endcsname{{\FAone\symbol{127}}}
\expandafter\def\csname faicon@mars-double\endcsname{{\FAone\symbol{128}}}
\expandafter\def\csname faicon@venus-mars\endcsname{{\FAone\symbol{129}}}
\expandafter\def\csname faicon@mars-stroke\endcsname{{\FAone\symbol{130}}}
\expandafter\def\csname faicon@mars-stroke-v\endcsname{{\FAone\symbol{131}}}
\expandafter\def\csname faicon@mars-stroke-h\endcsname{{\FAone\symbol{132}}}
\expandafter\def\csname faicon@neuter\endcsname{{\FAone\symbol{133}}}
\expandafter\def\csname faicon@genderless\endcsname{{\FAone\symbol{134}}}
\expandafter\def\csname faicon@facebook-official\endcsname{{\FAone\symbol{135}}}
\expandafter\def\csname faicon@pinterest-p\endcsname{{\FAone\symbol{136}}}
\expandafter\def\csname faicon@whatsapp\endcsname{{\FAone\symbol{137}}}
\expandafter\def\csname faicon@server\endcsname{{\FAone\symbol{138}}}
\expandafter\def\csname faicon@user-plus\endcsname{{\FAone\symbol{139}}}
\expandafter\def\csname faicon@user-times\endcsname{{\FAone\symbol{140}}}
\expandafter\def\csname faicon@bed\endcsname{{\FAone\symbol{141}}}
\expandafter\def\csname faicon@viacoin\endcsname{{\FAone\symbol{142}}}
\expandafter\def\csname faicon@train\endcsname{{\FAone\symbol{143}}}
\expandafter\def\csname faicon@subway\endcsname{{\FAone\symbol{144}}}
\expandafter\def\csname faicon@medium\endcsname{{\FAone\symbol{145}}}
\expandafter\def\csname faicon@y-combinator\endcsname{{\FAone\symbol{146}}}
\expandafter\def\csname faicon@optin-monster\endcsname{{\FAone\symbol{147}}}
\expandafter\def\csname faicon@opencart\endcsname{{\FAone\symbol{148}}}
\expandafter\def\csname faicon@expeditedssl\endcsname{{\FAone\symbol{149}}}
\expandafter\def\csname faicon@battery-full\endcsname{{\FAone\symbol{150}}}
\expandafter\def\csname faicon@battery-three-quarters\endcsname{{\FAone\symbol{151}}}
\expandafter\def\csname faicon@battery-half\endcsname{{\FAone\symbol{152}}}
\expandafter\def\csname faicon@battery-quarter\endcsname{{\FAone\symbol{153}}}
\expandafter\def\csname faicon@battery-empty\endcsname{{\FAone\symbol{154}}}
\expandafter\def\csname faicon@mouse-pointer\endcsname{{\FAone\symbol{155}}}
\expandafter\def\csname faicon@i-cursor\endcsname{{\FAone\symbol{156}}}
\expandafter\def\csname faicon@object-group\endcsname{{\FAone\symbol{157}}}
\expandafter\def\csname faicon@object-ungroup\endcsname{{\FAone\symbol{158}}}
\expandafter\def\csname faicon@sticky-note\endcsname{{\FAone\symbol{159}}}
\expandafter\def\csname faicon@sticky-note-o\endcsname{{\FAone\symbol{160}}}
\expandafter\def\csname faicon@cc-jcb\endcsname{{\FAone\symbol{161}}}
\expandafter\def\csname faicon@cc-diners-club\endcsname{{\FAone\symbol{162}}}
\expandafter\def\csname faicon@clone\endcsname{{\FAone\symbol{163}}}
\expandafter\def\csname faicon@balance-scale\endcsname{{\FAone\symbol{164}}}
\expandafter\def\csname faicon@hourglass-o\endcsname{{\FAone\symbol{165}}}
\expandafter\def\csname faicon@hourglass-start\endcsname{{\FAone\symbol{166}}}
\expandafter\def\csname faicon@hourglass-half\endcsname{{\FAone\symbol{167}}}
\expandafter\def\csname faicon@hourglass-end\endcsname{{\FAone\symbol{168}}}
\expandafter\def\csname faicon@hourglass\endcsname{{\FAone\symbol{169}}}
\expandafter\def\csname faicon@hand-rock-o\endcsname{{\FAone\symbol{170}}}
\expandafter\def\csname faicon@hand-paper-o\endcsname{{\FAone\symbol{171}}}
\expandafter\def\csname faicon@hand-scissors-o\endcsname{{\FAone\symbol{172}}}
\expandafter\def\csname faicon@hand-lizard-o\endcsname{{\FAone\symbol{173}}}
\expandafter\def\csname faicon@hand-spock-o\endcsname{{\FAone\symbol{174}}}
\expandafter\def\csname faicon@hand-pointer-o\endcsname{{\FAone\symbol{175}}}
\expandafter\def\csname faicon@hand-peace-o\endcsname{{\FAone\symbol{176}}}
\expandafter\def\csname faicon@trademark\endcsname{{\FAone\symbol{177}}}
\expandafter\def\csname faicon@registered\endcsname{{\FAone\symbol{178}}}
\expandafter\def\csname faicon@creative-commons\endcsname{{\FAone\symbol{179}}}
\expandafter\def\csname faicon@tripadvisor\endcsname{{\FAone\symbol{180}}}
\expandafter\def\csname faicon@odnoklassniki-square\endcsname{{\FAone\symbol{181}}}
\expandafter\def\csname faicon@get-pocket\endcsname{{\FAone\symbol{182}}}
\expandafter\def\csname faicon@wikipedia-w\endcsname{{\FAone\symbol{183}}}
\expandafter\def\csname faicon@safari\endcsname{{\FAone\symbol{184}}}
\expandafter\def\csname faicon@chrome\endcsname{{\FAone\symbol{185}}}
\expandafter\def\csname faicon@firefox\endcsname{{\FAone\symbol{186}}}
\expandafter\def\csname faicon@opera\endcsname{{\FAone\symbol{187}}}
\expandafter\def\csname faicon@internet-explorer\endcsname{{\FAone\symbol{188}}}
\expandafter\def\csname faicon@television\endcsname{{\FAone\symbol{189}}}
\expandafter\def\csname faicon@contao\endcsname{{\FAone\symbol{190}}}
\expandafter\def\csname faicon@500px\endcsname{{\FAone\symbol{191}}}
\expandafter\def\csname faicon@amazon\endcsname{{\FAone\symbol{192}}}
\expandafter\def\csname faicon@calendar-plus-o\endcsname{{\FAone\symbol{193}}}
\expandafter\def\csname faicon@calendar-minus-o\endcsname{{\FAone\symbol{194}}}
\expandafter\def\csname faicon@calendar-times-o\endcsname{{\FAone\symbol{195}}}
\expandafter\def\csname faicon@calendar-check-o\endcsname{{\FAone\symbol{196}}}
\expandafter\def\csname faicon@industry\endcsname{{\FAone\symbol{197}}}
\expandafter\def\csname faicon@map-pin\endcsname{{\FAone\symbol{198}}}
\expandafter\def\csname faicon@map-signs\endcsname{{\FAone\symbol{199}}}
\expandafter\def\csname faicon@map-o\endcsname{{\FAone\symbol{200}}}
\expandafter\def\csname faicon@map\endcsname{{\FAone\symbol{201}}}
\expandafter\def\csname faicon@commenting\endcsname{{\FAone\symbol{202}}}
\expandafter\def\csname faicon@commenting-o\endcsname{{\FAone\symbol{203}}}
\expandafter\def\csname faicon@houzz\endcsname{{\FAone\symbol{204}}}
\expandafter\def\csname faicon@vimeo\endcsname{{\FAone\symbol{205}}}
\expandafter\def\csname faicon@edge\endcsname{{\FAone\symbol{206}}}
\expandafter\def\csname faicon@credit-card-alt\endcsname{{\FAone\symbol{207}}}
\expandafter\def\csname faicon@codiepie\endcsname{{\FAone\symbol{208}}}
\expandafter\def\csname faicon@usb\endcsname{{\FAone\symbol{209}}}
\expandafter\def\csname faicon@product-hunt\endcsname{{\FAone\symbol{210}}}
\expandafter\def\csname faicon@mixcloud\endcsname{{\FAone\symbol{211}}}
\expandafter\def\csname faicon@scribd\endcsname{{\FAone\symbol{212}}}
\expandafter\def\csname faicon@pause-circle\endcsname{{\FAone\symbol{213}}}
\expandafter\def\csname faicon@pause-circle-o\endcsname{{\FAone\symbol{214}}}
\expandafter\def\csname faicon@stop-circle\endcsname{{\FAone\symbol{215}}}
\expandafter\def\csname faicon@stop-circle-o\endcsname{{\FAone\symbol{216}}}
\expandafter\def\csname faicon@shopping-bag\endcsname{{\FAone\symbol{217}}}
\expandafter\def\csname faicon@shopping-basket\endcsname{{\FAone\symbol{218}}}
\expandafter\def\csname faicon@hashtag\endcsname{{\FAone\symbol{219}}}
\expandafter\def\csname faicon@bluetooth\endcsname{{\FAone\symbol{220}}}
\expandafter\def\csname faicon@bluetooth-b\endcsname{{\FAone\symbol{221}}}
\expandafter\def\csname faicon@percent\endcsname{{\FAone\symbol{222}}}
\expandafter\def\csname faicon@gitlab\endcsname{{\FAone\symbol{223}}}
\expandafter\def\csname faicon@wpbeginner\endcsname{{\FAone\symbol{224}}}
\expandafter\def\csname faicon@wpforms\endcsname{{\FAone\symbol{225}}}
\expandafter\def\csname faicon@envira\endcsname{{\FAone\symbol{226}}}
\expandafter\def\csname faicon@universal-access\endcsname{{\FAone\symbol{227}}}
\expandafter\def\csname faicon@wheelchair-alt\endcsname{{\FAone\symbol{228}}}
\expandafter\def\csname faicon@question-circle-o\endcsname{{\FAone\symbol{229}}}
\expandafter\def\csname faicon@blind\endcsname{{\FAone\symbol{230}}}
\expandafter\def\csname faicon@audio-description\endcsname{{\FAone\symbol{231}}}
\expandafter\def\csname faicon@adjust\endcsname{{\FAone\symbol{232}}}
\expandafter\def\csname faicon@adn\endcsname{{\FAone\symbol{233}}}
\expandafter\def\csname faicon@align-center\endcsname{{\FAone\symbol{234}}}
\expandafter\def\csname faicon@align-justify\endcsname{{\FAone\symbol{235}}}
\expandafter\def\csname faicon@align-left\endcsname{{\FAone\symbol{236}}}
\expandafter\def\csname faicon@align-right\endcsname{{\FAone\symbol{237}}}
\expandafter\def\csname faicon@ambulance\endcsname{{\FAone\symbol{238}}}
\expandafter\def\csname faicon@anchor\endcsname{{\FAone\symbol{239}}}
\expandafter\def\csname faicon@android\endcsname{{\FAone\symbol{240}}}
\expandafter\def\csname faicon@angle-down\endcsname{{\FAone\symbol{241}}}
\expandafter\def\csname faicon@angle-left\endcsname{{\FAone\symbol{242}}}
\expandafter\def\csname faicon@angle-right\endcsname{{\FAone\symbol{243}}}
\expandafter\def\csname faicon@angle-up\endcsname{{\FAone\symbol{244}}}
\expandafter\def\csname faicon@apple\endcsname{{\FAone\symbol{245}}}
\expandafter\def\csname faicon@archive\endcsname{{\FAone\symbol{246}}}
\expandafter\def\csname faicon@arrow-circle-o-left\endcsname{{\FAone\symbol{247}}}
\expandafter\def\csname faicon@arrow-down\endcsname{{\FAone\symbol{248}}}
\expandafter\def\csname faicon@arrow-left\endcsname{{\FAone\symbol{249}}}
\expandafter\def\csname faicon@arrow-right\endcsname{{\FAone\symbol{250}}}
\expandafter\def\csname faicon@arrow-up\endcsname{{\FAone\symbol{251}}}
\expandafter\def\csname faicon@asterisk\endcsname{{\FAone\symbol{252}}}
\expandafter\def\csname faicon@backward\endcsname{{\FAone\symbol{253}}}
\expandafter\def\csname faicon@ban\endcsname{{\FAone\symbol{254}}}
\expandafter\def\csname faicon@bar-chart\endcsname{{\FAone\symbol{255}}}
\expandafter\def\csname faicon@barcode\endcsname{{\FAtwo\symbol{0}}}
\expandafter\def\csname faicon@flask\endcsname{{\FAtwo\symbol{1}}}
\expandafter\def\csname faicon@beer\endcsname{{\FAtwo\symbol{2}}}
\expandafter\def\csname faicon@bell-o\endcsname{{\FAtwo\symbol{3}}}
\expandafter\def\csname faicon@bell\endcsname{{\FAtwo\symbol{4}}}
\expandafter\def\csname faicon@bitbucket-square\endcsname{{\FAtwo\symbol{5}}}
\expandafter\def\csname faicon@bold\endcsname{{\FAtwo\symbol{6}}}
\expandafter\def\csname faicon@bolt\endcsname{{\FAtwo\symbol{7}}}
\expandafter\def\csname faicon@book\endcsname{{\FAtwo\symbol{8}}}
\expandafter\def\csname faicon@bookmark\endcsname{{\FAtwo\symbol{9}}}
\expandafter\def\csname faicon@bookmark-o\endcsname{{\FAtwo\symbol{10}}}
\expandafter\def\csname faicon@briefcase\endcsname{{\FAtwo\symbol{11}}}
\expandafter\def\csname faicon@btc\endcsname{{\FAtwo\symbol{12}}}
\expandafter\def\csname faicon@bug\endcsname{{\FAtwo\symbol{13}}}
\expandafter\def\csname faicon@building-o\endcsname{{\FAtwo\symbol{14}}}
\expandafter\def\csname faicon@bullhorn\endcsname{{\FAtwo\symbol{15}}}
\expandafter\def\csname faicon@bullseye\endcsname{{\FAtwo\symbol{16}}}
\expandafter\def\csname faicon@calendar\endcsname{{\FAtwo\symbol{17}}}
\expandafter\def\csname faicon@calendar-o\endcsname{{\FAtwo\symbol{18}}}
\expandafter\def\csname faicon@camera\endcsname{{\FAtwo\symbol{19}}}
\expandafter\def\csname faicon@camera-retro\endcsname{{\FAtwo\symbol{20}}}
\expandafter\def\csname faicon@caret-down\endcsname{{\FAtwo\symbol{21}}}
\expandafter\def\csname faicon@caret-left\endcsname{{\FAtwo\symbol{22}}}
\expandafter\def\csname faicon@caret-right\endcsname{{\FAtwo\symbol{23}}}
\expandafter\def\csname faicon@caret-up\endcsname{{\FAtwo\symbol{24}}}
\expandafter\def\csname faicon@certificate\endcsname{{\FAtwo\symbol{25}}}
\expandafter\def\csname faicon@check-square-o\endcsname{{\FAtwo\symbol{26}}}
\expandafter\def\csname faicon@square-o\endcsname{{\FAtwo\symbol{27}}}
\expandafter\def\csname faicon@minus-square-o\endcsname{{\FAtwo\symbol{28}}}
\expandafter\def\csname faicon@check-square\endcsname{{\FAtwo\symbol{29}}}
\expandafter\def\csname faicon@chevron-down\endcsname{{\FAtwo\symbol{30}}}
\expandafter\def\csname faicon@chevron-left\endcsname{{\FAtwo\symbol{31}}}
\expandafter\def\csname faicon@chevron-right\endcsname{{\FAtwo\symbol{32}}}
\expandafter\def\csname faicon@chevron-circle-down\endcsname{{\FAtwo\symbol{33}}}
\expandafter\def\csname faicon@chevron-circle-left\endcsname{{\FAtwo\symbol{34}}}
\expandafter\def\csname faicon@chevron-circle-right\endcsname{{\FAtwo\symbol{35}}}
\expandafter\def\csname faicon@chevron-circle-up\endcsname{{\FAtwo\symbol{36}}}
\expandafter\def\csname faicon@chevron-up\endcsname{{\FAtwo\symbol{37}}}
\expandafter\def\csname faicon@circle\endcsname{{\FAtwo\symbol{38}}}
\expandafter\def\csname faicon@arrow-circle-down\endcsname{{\FAtwo\symbol{39}}}
\expandafter\def\csname faicon@arrow-circle-left\endcsname{{\FAtwo\symbol{40}}}
\expandafter\def\csname faicon@arrow-circle-right\endcsname{{\FAtwo\symbol{41}}}
\expandafter\def\csname faicon@arrow-circle-up\endcsname{{\FAtwo\symbol{42}}}
\expandafter\def\csname faicon@circle-o\endcsname{{\FAtwo\symbol{43}}}
\expandafter\def\csname faicon@cloud\endcsname{{\FAtwo\symbol{44}}}
\expandafter\def\csname faicon@cloud-download\endcsname{{\FAtwo\symbol{45}}}
\expandafter\def\csname faicon@cloud-upload\endcsname{{\FAtwo\symbol{46}}}
\expandafter\def\csname faicon@code\endcsname{{\FAtwo\symbol{47}}}
\expandafter\def\csname faicon@code-fork\endcsname{{\FAtwo\symbol{48}}}
\expandafter\def\csname faicon@coffee\endcsname{{\FAtwo\symbol{49}}}
\expandafter\def\csname faicon@cog\endcsname{{\FAtwo\symbol{50}}}
\expandafter\def\csname faicon@cogs\endcsname{{\FAtwo\symbol{51}}}
\expandafter\def\csname faicon@caret-square-o-down\endcsname{{\FAtwo\symbol{52}}}
\expandafter\def\csname faicon@caret-square-o-up\endcsname{{\FAtwo\symbol{53}}}
\expandafter\def\csname faicon@columns\endcsname{{\FAtwo\symbol{54}}}
\expandafter\def\csname faicon@comment\endcsname{{\FAtwo\symbol{55}}}
\expandafter\def\csname faicon@comment-o\endcsname{{\FAtwo\symbol{56}}}
\expandafter\def\csname faicon@comments\endcsname{{\FAtwo\symbol{57}}}
\expandafter\def\csname faicon@comments-o\endcsname{{\FAtwo\symbol{58}}}
\expandafter\def\csname faicon@compass\endcsname{{\FAtwo\symbol{59}}}
\expandafter\def\csname faicon@files-o\endcsname{{\FAtwo\symbol{60}}}
\expandafter\def\csname faicon@credit-card\endcsname{{\FAtwo\symbol{61}}}
\expandafter\def\csname faicon@crop\endcsname{{\FAtwo\symbol{62}}}
\expandafter\def\csname faicon@css3\endcsname{{\FAtwo\symbol{63}}}
\expandafter\def\csname faicon@scissors\endcsname{{\FAtwo\symbol{64}}}
\expandafter\def\csname faicon@tachometer\endcsname{{\FAtwo\symbol{65}}}
\expandafter\def\csname faicon@desktop\endcsname{{\FAtwo\symbol{66}}}
\expandafter\def\csname faicon@dot-circle-o\endcsname{{\FAtwo\symbol{67}}}
\expandafter\def\csname faicon@angle-double-down\endcsname{{\FAtwo\symbol{68}}}
\expandafter\def\csname faicon@angle-double-left\endcsname{{\FAtwo\symbol{69}}}
\expandafter\def\csname faicon@angle-double-right\endcsname{{\FAtwo\symbol{70}}}
\expandafter\def\csname faicon@angle-double-up\endcsname{{\FAtwo\symbol{71}}}
\expandafter\def\csname faicon@arrow-circle-o-down\endcsname{{\FAtwo\symbol{72}}}
\expandafter\def\csname faicon@download\endcsname{{\FAtwo\symbol{73}}}
\expandafter\def\csname faicon@dribbble\endcsname{{\FAtwo\symbol{74}}}
\expandafter\def\csname faicon@dropbox\endcsname{{\FAtwo\symbol{75}}}
\expandafter\def\csname faicon@pencil-square-o\endcsname{{\FAtwo\symbol{76}}}
\expandafter\def\csname faicon@pencil-square\endcsname{{\FAtwo\symbol{77}}}
\expandafter\def\csname faicon@eject\endcsname{{\FAtwo\symbol{78}}}
\expandafter\def\csname faicon@ellipsis-h\endcsname{{\FAtwo\symbol{79}}}
\expandafter\def\csname faicon@ellipsis-v\endcsname{{\FAtwo\symbol{80}}}
\expandafter\def\csname faicon@envelope-o\endcsname{{\FAtwo\symbol{81}}}
\expandafter\def\csname faicon@envelope\endcsname{{\FAtwo\symbol{82}}}
\expandafter\def\csname faicon@eur\endcsname{{\FAtwo\symbol{83}}}
\expandafter\def\csname faicon@exchange\endcsname{{\FAtwo\symbol{84}}}
\expandafter\def\csname faicon@exclamation\endcsname{{\FAtwo\symbol{85}}}
\expandafter\def\csname faicon@exclamation-circle\endcsname{{\FAtwo\symbol{86}}}
\expandafter\def\csname faicon@external-link\endcsname{{\FAtwo\symbol{87}}}
\expandafter\def\csname faicon@eye-slash\endcsname{{\FAtwo\symbol{88}}}
\expandafter\def\csname faicon@eye\endcsname{{\FAtwo\symbol{89}}}
\expandafter\def\csname faicon@plus-square\endcsname{{\FAtwo\symbol{90}}}
\expandafter\def\csname faicon@bitbucket\endcsname{{\FAtwo\symbol{91}}}
\expandafter\def\csname faicon@reddit\endcsname{{\FAtwo\symbol{92}}}
\expandafter\def\csname faicon@stumbleupon\endcsname{{\FAtwo\symbol{93}}}
\expandafter\def\csname faicon@language\endcsname{{\FAtwo\symbol{94}}}
\expandafter\def\csname faicon@cc-amex\endcsname{{\FAtwo\symbol{95}}}
\expandafter\def\csname faicon@paint-brush\endcsname{{\FAtwo\symbol{96}}}
\expandafter\def\csname faicon@dashcube\endcsname{{\FAtwo\symbol{97}}}
\expandafter\def\csname faicon@leanpub\endcsname{{\FAtwo\symbol{98}}}
\expandafter\def\csname faicon@gg\endcsname{{\FAtwo\symbol{99}}}
\expandafter\def\csname faicon@gg-circle\endcsname{{\FAtwo\symbol{100}}}
\expandafter\def\csname faicon@odnoklassniki\endcsname{{\FAtwo\symbol{101}}}
\expandafter\def\csname faicon@black-tie\endcsname{{\FAtwo\symbol{102}}}
\expandafter\def\csname faicon@facebook\endcsname{{\FAtwo\symbol{103}}}
\expandafter\def\csname faicon@facebook-square\endcsname{{\FAtwo\symbol{104}}}
\expandafter\def\csname faicon@video-camera\endcsname{{\FAtwo\symbol{105}}}
\expandafter\def\csname faicon@fast-backward\endcsname{{\FAtwo\symbol{106}}}
\expandafter\def\csname faicon@fast-forward\endcsname{{\FAtwo\symbol{107}}}
\expandafter\def\csname faicon@female\endcsname{{\FAtwo\symbol{108}}}
\expandafter\def\csname faicon@fighter-jet\endcsname{{\FAtwo\symbol{109}}}
\expandafter\def\csname faicon@file\endcsname{{\FAtwo\symbol{110}}}
\expandafter\def\csname faicon@file-o\endcsname{{\FAtwo\symbol{111}}}
\expandafter\def\csname faicon@file-text\endcsname{{\FAtwo\symbol{112}}}
\expandafter\def\csname faicon@file-text-o\endcsname{{\FAtwo\symbol{113}}}
\expandafter\def\csname faicon@film\endcsname{{\FAtwo\symbol{114}}}
\expandafter\def\csname faicon@filter\endcsname{{\FAtwo\symbol{115}}}
\expandafter\def\csname faicon@fire\endcsname{{\FAtwo\symbol{116}}}
\expandafter\def\csname faicon@fire-extinguisher\endcsname{{\FAtwo\symbol{117}}}
\expandafter\def\csname faicon@flag\endcsname{{\FAtwo\symbol{118}}}
\expandafter\def\csname faicon@flag-o\endcsname{{\FAtwo\symbol{119}}}
\expandafter\def\csname faicon@flag-checkered\endcsname{{\FAtwo\symbol{120}}}
\expandafter\def\csname faicon@flickr\endcsname{{\FAtwo\symbol{121}}}
\expandafter\def\csname faicon@folder\endcsname{{\FAtwo\symbol{122}}}
\expandafter\def\csname faicon@folder-o\endcsname{{\FAtwo\symbol{123}}}
\expandafter\def\csname faicon@folder-open\endcsname{{\FAtwo\symbol{124}}}
\expandafter\def\csname faicon@folder-open-o\endcsname{{\FAtwo\symbol{125}}}
\expandafter\def\csname faicon@font\endcsname{{\FAtwo\symbol{126}}}
\expandafter\def\csname faicon@cutlery\endcsname{{\FAtwo\symbol{127}}}
\expandafter\def\csname faicon@forward\endcsname{{\FAtwo\symbol{128}}}
\expandafter\def\csname faicon@foursquare\endcsname{{\FAtwo\symbol{129}}}
\expandafter\def\csname faicon@frown-o\endcsname{{\FAtwo\symbol{130}}}
\expandafter\def\csname faicon@arrows-alt\endcsname{{\FAtwo\symbol{131}}}
\expandafter\def\csname faicon@gamepad\endcsname{{\FAtwo\symbol{132}}}
\expandafter\def\csname faicon@gbp\endcsname{{\FAtwo\symbol{133}}}
\expandafter\def\csname faicon@gift\endcsname{{\FAtwo\symbol{134}}}
\expandafter\def\csname faicon@github\endcsname{{\FAtwo\symbol{135}}}
\expandafter\def\csname faicon@github-alt\endcsname{{\FAtwo\symbol{136}}}
\expandafter\def\csname faicon@github-square\endcsname{{\FAtwo\symbol{137}}}
\expandafter\def\csname faicon@gratipay\endcsname{{\FAtwo\symbol{138}}}
\expandafter\def\csname faicon@glass\endcsname{{\FAtwo\symbol{139}}}
\expandafter\def\csname faicon@globe\endcsname{{\FAtwo\symbol{140}}}
\expandafter\def\csname faicon@google-plus\endcsname{{\FAtwo\symbol{141}}}
\expandafter\def\csname faicon@google-plus-square\endcsname{{\FAtwo\symbol{142}}}
\expandafter\def\csname faicon@users\endcsname{{\FAtwo\symbol{143}}}
\expandafter\def\csname faicon@h-square\endcsname{{\FAtwo\symbol{144}}}
\expandafter\def\csname faicon@hand-o-down\endcsname{{\FAtwo\symbol{145}}}
\expandafter\def\csname faicon@hand-o-left\endcsname{{\FAtwo\symbol{146}}}
\expandafter\def\csname faicon@hand-o-right\endcsname{{\FAtwo\symbol{147}}}
\expandafter\def\csname faicon@hand-o-up\endcsname{{\FAtwo\symbol{148}}}
\expandafter\def\csname faicon@hdd-o\endcsname{{\FAtwo\symbol{149}}}
\expandafter\def\csname faicon@headphones\endcsname{{\FAtwo\symbol{150}}}
\expandafter\def\csname faicon@heart\endcsname{{\FAtwo\symbol{151}}}
\expandafter\def\csname faicon@heart-o\endcsname{{\FAtwo\symbol{152}}}
\expandafter\def\csname faicon@home\endcsname{{\FAtwo\symbol{153}}}
\expandafter\def\csname faicon@hospital-o\endcsname{{\FAtwo\symbol{154}}}
\expandafter\def\csname faicon@html5\endcsname{{\FAtwo\symbol{155}}}
\expandafter\def\csname faicon@inbox\endcsname{{\FAtwo\symbol{156}}}
\expandafter\def\csname faicon@outdent\endcsname{{\FAtwo\symbol{157}}}
\expandafter\def\csname faicon@indent\endcsname{{\FAtwo\symbol{158}}}
\expandafter\def\csname faicon@info-circle\endcsname{{\FAtwo\symbol{159}}}
\expandafter\def\csname faicon@inr\endcsname{{\FAtwo\symbol{160}}}
\expandafter\def\csname faicon@instagram\endcsname{{\FAtwo\symbol{161}}}
\expandafter\def\csname faicon@italic\endcsname{{\FAtwo\symbol{162}}}
\expandafter\def\csname faicon@jpy\endcsname{{\FAtwo\symbol{163}}}
\expandafter\def\csname faicon@key\endcsname{{\FAtwo\symbol{164}}}
\expandafter\def\csname faicon@keyboard-o\endcsname{{\FAtwo\symbol{165}}}
\expandafter\def\csname faicon@krw\endcsname{{\FAtwo\symbol{166}}}
\expandafter\def\csname faicon@laptop\endcsname{{\FAtwo\symbol{167}}}
\expandafter\def\csname faicon@leaf\endcsname{{\FAtwo\symbol{168}}}
\expandafter\def\csname faicon@gavel\endcsname{{\FAtwo\symbol{169}}}
\expandafter\def\csname faicon@lemon-o\endcsname{{\FAtwo\symbol{170}}}
\expandafter\def\csname faicon@level-down\endcsname{{\FAtwo\symbol{171}}}
\expandafter\def\csname faicon@level-up\endcsname{{\FAtwo\symbol{172}}}
\expandafter\def\csname faicon@lightbulb-o\endcsname{{\FAtwo\symbol{173}}}
\expandafter\def\csname faicon@link\endcsname{{\FAtwo\symbol{174}}}
\expandafter\def\csname faicon@linkedin\endcsname{{\FAtwo\symbol{175}}}
\expandafter\def\csname faicon@linkedin-square\endcsname{{\FAtwo\symbol{176}}}
\expandafter\def\csname faicon@linux\endcsname{{\FAtwo\symbol{177}}}
\expandafter\def\csname faicon@list\endcsname{{\FAtwo\symbol{178}}}
\expandafter\def\csname faicon@list-alt\endcsname{{\FAtwo\symbol{179}}}
\expandafter\def\csname faicon@location-arrow\endcsname{{\FAtwo\symbol{180}}}
\expandafter\def\csname faicon@lock\endcsname{{\FAtwo\symbol{181}}}
\expandafter\def\csname faicon@long-arrow-down\endcsname{{\FAtwo\symbol{182}}}
\expandafter\def\csname faicon@long-arrow-left\endcsname{{\FAtwo\symbol{183}}}
\expandafter\def\csname faicon@long-arrow-right\endcsname{{\FAtwo\symbol{184}}}
\expandafter\def\csname faicon@long-arrow-up\endcsname{{\FAtwo\symbol{185}}}
\expandafter\def\csname faicon@magic\endcsname{{\FAtwo\symbol{186}}}
\expandafter\def\csname faicon@magnet\endcsname{{\FAtwo\symbol{187}}}
\expandafter\def\csname faicon@male\endcsname{{\FAtwo\symbol{188}}}
\expandafter\def\csname faicon@map-marker\endcsname{{\FAtwo\symbol{189}}}
\expandafter\def\csname faicon@maxcdn\endcsname{{\FAtwo\symbol{190}}}
\expandafter\def\csname faicon@medkit\endcsname{{\FAtwo\symbol{191}}}
\expandafter\def\csname faicon@meh-o\endcsname{{\FAtwo\symbol{192}}}
\expandafter\def\csname faicon@microphone\endcsname{{\FAtwo\symbol{193}}}
\expandafter\def\csname faicon@microphone-slash\endcsname{{\FAtwo\symbol{194}}}
\expandafter\def\csname faicon@minus\endcsname{{\FAtwo\symbol{195}}}
\expandafter\def\csname faicon@minus-circle\endcsname{{\FAtwo\symbol{196}}}
\expandafter\def\csname faicon@minus-square\endcsname{{\FAtwo\symbol{197}}}
\expandafter\def\csname faicon@mobile\endcsname{{\FAtwo\symbol{198}}}
\expandafter\def\csname faicon@money\endcsname{{\FAtwo\symbol{199}}}
\expandafter\def\csname faicon@arrows\endcsname{{\FAtwo\symbol{200}}}
\expandafter\def\csname faicon@music\endcsname{{\FAtwo\symbol{201}}}
\expandafter\def\csname faicon@power-off\endcsname{{\FAtwo\symbol{202}}}
\expandafter\def\csname faicon@check\endcsname{{\FAtwo\symbol{203}}}
\expandafter\def\csname faicon@check-circle-o\endcsname{{\FAtwo\symbol{204}}}
\expandafter\def\csname faicon@check-circle\endcsname{{\FAtwo\symbol{205}}}
\expandafter\def\csname faicon@list-ol\endcsname{{\FAtwo\symbol{206}}}
\expandafter\def\csname faicon@paperclip\endcsname{{\FAtwo\symbol{207}}}
\expandafter\def\csname faicon@clipboard\endcsname{{\FAtwo\symbol{208}}}
\expandafter\def\csname faicon@pause\endcsname{{\FAtwo\symbol{209}}}
\expandafter\def\csname faicon@pencil\endcsname{{\FAtwo\symbol{210}}}
\expandafter\def\csname faicon@phone\endcsname{{\FAtwo\symbol{211}}}
\expandafter\def\csname faicon@phone-square\endcsname{{\FAtwo\symbol{212}}}
\expandafter\def\csname faicon@picture-o\endcsname{{\FAtwo\symbol{213}}}
\expandafter\def\csname faicon@pinterest\endcsname{{\FAtwo\symbol{214}}}
\expandafter\def\csname faicon@pinterest-square\endcsname{{\FAtwo\symbol{215}}}
\expandafter\def\csname faicon@plane\endcsname{{\FAtwo\symbol{216}}}
\expandafter\def\csname faicon@play\endcsname{{\FAtwo\symbol{217}}}
\expandafter\def\csname faicon@play-circle-o\endcsname{{\FAtwo\symbol{218}}}
\expandafter\def\csname faicon@play-circle\endcsname{{\FAtwo\symbol{219}}}
\expandafter\def\csname faicon@plus\endcsname{{\FAtwo\symbol{220}}}
\expandafter\def\csname faicon@plus-circle\endcsname{{\FAtwo\symbol{221}}}
\expandafter\def\csname faicon@plus-square-o\endcsname{{\FAtwo\symbol{222}}}
\expandafter\def\csname faicon@print\endcsname{{\FAtwo\symbol{223}}}
\expandafter\def\csname faicon@thumb-tack\endcsname{{\FAtwo\symbol{224}}}
\expandafter\def\csname faicon@puzzle-piece\endcsname{{\FAtwo\symbol{225}}}
\expandafter\def\csname faicon@qrcode\endcsname{{\FAtwo\symbol{226}}}
\expandafter\def\csname faicon@question\endcsname{{\FAtwo\symbol{227}}}
\expandafter\def\csname faicon@question-circle\endcsname{{\FAtwo\symbol{228}}}
\expandafter\def\csname faicon@quote-left\endcsname{{\FAtwo\symbol{229}}}
\expandafter\def\csname faicon@quote-right\endcsname{{\FAtwo\symbol{230}}}
\expandafter\def\csname faicon@random\endcsname{{\FAtwo\symbol{231}}}
\expandafter\def\csname faicon@refresh\endcsname{{\FAtwo\symbol{232}}}
\expandafter\def\csname faicon@times\endcsname{{\FAtwo\symbol{233}}}
\expandafter\def\csname faicon@times-circle-o\endcsname{{\FAtwo\symbol{234}}}
\expandafter\def\csname faicon@times-circle\endcsname{{\FAtwo\symbol{235}}}
\expandafter\def\csname faicon@renren\endcsname{{\FAtwo\symbol{236}}}
\expandafter\def\csname faicon@bars\endcsname{{\FAtwo\symbol{237}}}
\expandafter\def\csname faicon@repeat\endcsname{{\FAtwo\symbol{238}}}
\expandafter\def\csname faicon@reply\endcsname{{\FAtwo\symbol{239}}}
\expandafter\def\csname faicon@reply-all\endcsname{{\FAtwo\symbol{240}}}
\expandafter\def\csname faicon@expand\endcsname{{\FAtwo\symbol{241}}}
\expandafter\def\csname faicon@arrows-h\endcsname{{\FAtwo\symbol{242}}}
\expandafter\def\csname faicon@compress\endcsname{{\FAtwo\symbol{243}}}
\expandafter\def\csname faicon@arrows-v\endcsname{{\FAtwo\symbol{244}}}
\expandafter\def\csname faicon@retweet\endcsname{{\FAtwo\symbol{245}}}
\expandafter\def\csname faicon@road\endcsname{{\FAtwo\symbol{246}}}
\expandafter\def\csname faicon@rocket\endcsname{{\FAtwo\symbol{247}}}
\expandafter\def\csname faicon@rss\endcsname{{\FAtwo\symbol{248}}}
\expandafter\def\csname faicon@rub\endcsname{{\FAtwo\symbol{249}}}
\expandafter\def\csname faicon@floppy-o\endcsname{{\FAtwo\symbol{250}}}
\expandafter\def\csname faicon@crosshairs\endcsname{{\FAtwo\symbol{251}}}
\expandafter\def\csname faicon@search\endcsname{{\FAtwo\symbol{252}}}
\expandafter\def\csname faicon@share-square-o\endcsname{{\FAtwo\symbol{253}}}
\expandafter\def\csname faicon@share\endcsname{{\FAtwo\symbol{254}}}
\expandafter\def\csname faicon@share-square\endcsname{{\FAtwo\symbol{255}}}
\expandafter\def\csname faicon@shield\endcsname{{\FAthree\symbol{0}}}
\expandafter\def\csname faicon@shopping-cart\endcsname{{\FAthree\symbol{1}}}
\expandafter\def\csname faicon@square\endcsname{{\FAthree\symbol{2}}}
\expandafter\def\csname faicon@signal\endcsname{{\FAthree\symbol{3}}}
\expandafter\def\csname faicon@sign-in\endcsname{{\FAthree\symbol{4}}}
\expandafter\def\csname faicon@sign-out\endcsname{{\FAthree\symbol{5}}}
\expandafter\def\csname faicon@sitemap\endcsname{{\FAthree\symbol{6}}}
\expandafter\def\csname faicon@skype\endcsname{{\FAthree\symbol{7}}}
\expandafter\def\csname faicon@smile-o\endcsname{{\FAthree\symbol{8}}}
\expandafter\def\csname faicon@sort\endcsname{{\FAthree\symbol{9}}}
\expandafter\def\csname faicon@sort-alpha-asc\endcsname{{\FAthree\symbol{10}}}
\expandafter\def\csname faicon@sort-amount-asc\endcsname{{\FAthree\symbol{11}}}
\expandafter\def\csname faicon@sort-amount-desc\endcsname{{\FAthree\symbol{12}}}
\expandafter\def\csname faicon@sort-numeric-asc\endcsname{{\FAthree\symbol{13}}}
\expandafter\def\csname faicon@sort-numeric-desc\endcsname{{\FAthree\symbol{14}}}
\expandafter\def\csname faicon@sort-desc\endcsname{{\FAthree\symbol{15}}}
\expandafter\def\csname faicon@sort-asc\endcsname{{\FAthree\symbol{16}}}
\expandafter\def\csname faicon@spinner\endcsname{{\FAthree\symbol{17}}}
\expandafter\def\csname faicon@stack-exchange\endcsname{{\FAthree\symbol{18}}}
\expandafter\def\csname faicon@stack-overflow\endcsname{{\FAthree\symbol{19}}}
\expandafter\def\csname faicon@star\endcsname{{\FAthree\symbol{20}}}
\expandafter\def\csname faicon@star-o\endcsname{{\FAthree\symbol{21}}}
\expandafter\def\csname faicon@star-half\endcsname{{\FAthree\symbol{22}}}
\expandafter\def\csname faicon@star-half-o\endcsname{{\FAthree\symbol{23}}}
\expandafter\def\csname faicon@step-backward\endcsname{{\FAthree\symbol{24}}}
\expandafter\def\csname faicon@step-forward\endcsname{{\FAthree\symbol{25}}}
\expandafter\def\csname faicon@stethoscope\endcsname{{\FAthree\symbol{26}}}
\expandafter\def\csname faicon@stop\endcsname{{\FAthree\symbol{27}}}
\expandafter\def\csname faicon@strikethrough\endcsname{{\FAthree\symbol{28}}}
\expandafter\def\csname faicon@subscript\endcsname{{\FAthree\symbol{29}}}
\expandafter\def\csname faicon@suitcase\endcsname{{\FAthree\symbol{30}}}
\expandafter\def\csname faicon@sun-o\endcsname{{\FAthree\symbol{31}}}
\expandafter\def\csname faicon@superscript\endcsname{{\FAthree\symbol{32}}}
\expandafter\def\csname faicon@table\endcsname{{\FAthree\symbol{33}}}
\expandafter\def\csname faicon@tablet\endcsname{{\FAthree\symbol{34}}}
\expandafter\def\csname faicon@tag\endcsname{{\FAthree\symbol{35}}}
\expandafter\def\csname faicon@tags\endcsname{{\FAthree\symbol{36}}}
\expandafter\def\csname faicon@tasks\endcsname{{\FAthree\symbol{37}}}
\expandafter\def\csname faicon@terminal\endcsname{{\FAthree\symbol{38}}}
\expandafter\def\csname faicon@text-height\endcsname{{\FAthree\symbol{39}}}
\expandafter\def\csname faicon@text-width\endcsname{{\FAthree\symbol{40}}}
\expandafter\def\csname faicon@th\endcsname{{\FAthree\symbol{41}}}
\expandafter\def\csname faicon@th-large\endcsname{{\FAthree\symbol{42}}}
\expandafter\def\csname faicon@th-list\endcsname{{\FAthree\symbol{43}}}
\expandafter\def\csname faicon@thumbs-o-down\endcsname{{\FAthree\symbol{44}}}
\expandafter\def\csname faicon@thumbs-o-up\endcsname{{\FAthree\symbol{45}}}
\expandafter\def\csname faicon@ticket\endcsname{{\FAthree\symbol{46}}}
\expandafter\def\csname faicon@clock-o\endcsname{{\FAthree\symbol{47}}}
\expandafter\def\csname faicon@tint\endcsname{{\FAthree\symbol{48}}}
\expandafter\def\csname faicon@trash-o\endcsname{{\FAthree\symbol{49}}}
\expandafter\def\csname faicon@trello\endcsname{{\FAthree\symbol{50}}}
\expandafter\def\csname faicon@trophy\endcsname{{\FAthree\symbol{51}}}
\expandafter\def\csname faicon@truck\endcsname{{\FAthree\symbol{52}}}
\expandafter\def\csname faicon@tumblr\endcsname{{\FAthree\symbol{53}}}
\expandafter\def\csname faicon@tumblr-square\endcsname{{\FAthree\symbol{54}}}
\expandafter\def\csname faicon@twitter\endcsname{{\FAthree\symbol{55}}}
\expandafter\def\csname faicon@twitter-square\endcsname{{\FAthree\symbol{56}}}
\expandafter\def\csname faicon@list-ul\endcsname{{\FAthree\symbol{57}}}
\expandafter\def\csname faicon@umbrella\endcsname{{\FAthree\symbol{58}}}
\expandafter\def\csname faicon@underline\endcsname{{\FAthree\symbol{59}}}
\expandafter\def\csname faicon@undo\endcsname{{\FAthree\symbol{60}}}
\expandafter\def\csname faicon@google\endcsname{{\FAthree\symbol{61}}}
\expandafter\def\csname faicon@paw\endcsname{{\FAthree\symbol{62}}}
\expandafter\def\csname faicon@database\endcsname{{\FAthree\symbol{63}}}
\expandafter\def\csname faicon@file-pdf-o\endcsname{{\FAthree\symbol{64}}}
\expandafter\def\csname faicon@rebel\endcsname{{\FAthree\symbol{65}}}
\expandafter\def\csname faicon@empire\endcsname{{\FAthree\symbol{66}}}
\expandafter\def\csname faicon@git-square\endcsname{{\FAthree\symbol{67}}}
\expandafter\def\csname faicon@tencent-weibo\endcsname{{\FAthree\symbol{68}}}
\expandafter\def\csname faicon@qq\endcsname{{\FAthree\symbol{69}}}
\expandafter\def\csname faicon@weixin\endcsname{{\FAthree\symbol{70}}}
\expandafter\def\csname faicon@share-alt\endcsname{{\FAthree\symbol{71}}}
\expandafter\def\csname faicon@cc-visa\endcsname{{\FAthree\symbol{72}}}
\expandafter\def\csname faicon@fonticons\endcsname{{\FAthree\symbol{73}}}
\expandafter\def\csname faicon@reddit-alien\endcsname{{\FAthree\symbol{74}}}
\expandafter\def\csname faicon@modx\endcsname{{\FAthree\symbol{75}}}
\expandafter\def\csname faicon@fort-awesome\endcsname{{\FAthree\symbol{76}}}
\expandafter\def\csname faicon@volume-control-phone\endcsname{{\FAthree\symbol{77}}}
\expandafter\def\csname faicon@braille\endcsname{{\FAthree\symbol{78}}}
\expandafter\def\csname faicon@assistive-listening-systems\endcsname{{\FAthree\symbol{79}}}
\expandafter\def\csname faicon@american-sign-language-interpreting\endcsname{{\FAthree\symbol{80}}}
\expandafter\def\csname faicon@deaf\endcsname{{\FAthree\symbol{81}}}
\expandafter\def\csname faicon@glide\endcsname{{\FAthree\symbol{82}}}
\expandafter\def\csname faicon@glide-g\endcsname{{\FAthree\symbol{83}}}
\expandafter\def\csname faicon@sign-language\endcsname{{\FAthree\symbol{84}}}
\expandafter\def\csname faicon@low-vision\endcsname{{\FAthree\symbol{85}}}
\expandafter\def\csname faicon@viadeo\endcsname{{\FAthree\symbol{86}}}
\expandafter\def\csname faicon@viadeo-square\endcsname{{\FAthree\symbol{87}}}
\expandafter\def\csname faicon@snapchat\endcsname{{\FAthree\symbol{88}}}
\expandafter\def\csname faicon@snapchat-ghost\endcsname{{\FAthree\symbol{89}}}
\expandafter\def\csname faicon@snapchat-square\endcsname{{\FAthree\symbol{90}}}
\expandafter\def\csname faicon@pied-piper\endcsname{{\FAthree\symbol{91}}}
\expandafter\def\csname faicon@first-order\endcsname{{\FAthree\symbol{92}}}
\expandafter\def\csname faicon@yoast\endcsname{{\FAthree\symbol{93}}}
\expandafter\def\csname faicon@themeisle\endcsname{{\FAthree\symbol{94}}}
\expandafter\def\csname faicon@google-plus-official\endcsname{{\FAthree\symbol{95}}}
\expandafter\def\csname faicon@font-awesome\endcsname{{\FAthree\symbol{96}}}
\expandafter\def\csname faicon@chain-broken\endcsname{{\FAthree\symbol{97}}}
\expandafter\def\csname faicon@unlock\endcsname{{\FAthree\symbol{98}}}
\expandafter\def\csname faicon@unlock-alt\endcsname{{\FAthree\symbol{99}}}
\expandafter\def\csname faicon@arrow-circle-o-up\endcsname{{\FAthree\symbol{100}}}
\expandafter\def\csname faicon@upload\endcsname{{\FAthree\symbol{101}}}
\expandafter\def\csname faicon@usd\endcsname{{\FAthree\symbol{102}}}
\expandafter\def\csname faicon@user\endcsname{{\FAthree\symbol{103}}}
\expandafter\def\csname faicon@user-md\endcsname{{\FAthree\symbol{104}}}
\expandafter\def\csname faicon@venus\endcsname{{\FAthree\symbol{105}}}
\expandafter\def\csname faicon@vimeo-square\endcsname{{\FAthree\symbol{106}}}
\expandafter\def\csname faicon@vk\endcsname{{\FAthree\symbol{107}}}
\expandafter\def\csname faicon@volume-down\endcsname{{\FAthree\symbol{108}}}
\expandafter\def\csname faicon@volume-off\endcsname{{\FAthree\symbol{109}}}
\expandafter\def\csname faicon@volume-up\endcsname{{\FAthree\symbol{110}}}
\expandafter\def\csname faicon@exclamation-triangle\endcsname{{\FAthree\symbol{111}}}
\expandafter\def\csname faicon@weibo\endcsname{{\FAthree\symbol{112}}}
\expandafter\def\csname faicon@windows\endcsname{{\FAthree\symbol{113}}}
\expandafter\def\csname faicon@wrench\endcsname{{\FAthree\symbol{114}}}
\expandafter\def\csname faicon@xing\endcsname{{\FAthree\symbol{115}}}
\expandafter\def\csname faicon@xing-square\endcsname{{\FAthree\symbol{116}}}
\expandafter\def\csname faicon@youtube\endcsname{{\FAthree\symbol{117}}}
\expandafter\def\csname faicon@youtube-play\endcsname{{\FAthree\symbol{118}}}
\expandafter\def\csname faicon@youtube-square\endcsname{{\FAthree\symbol{119}}}
\expandafter\def\csname faicon@search-plus\endcsname{{\FAthree\symbol{120}}}
\expandafter\def\csname faicon@search-minus\endcsname{{\FAthree\symbol{121}}}

%% end of file `fontawesomesymbols-pdftex.tex'.


==> fontawesomesymbols-xeluatex.tex <==
\expandafter\def\csname faicon@glass\endcsname{{\FA\symbol{"F000}}}
\expandafter\def\csname faicon@music\endcsname{{\FA\symbol{"F001}}}
\expandafter\def\csname faicon@search\endcsname{{\FA\symbol{"F002}}}
\expandafter\def\csname faicon@envelope-o\endcsname{{\FA\symbol{"F003}}}
\expandafter\def\csname faicon@heart\endcsname{{\FA\symbol{"F004}}}
\expandafter\def\csname faicon@star\endcsname{{\FA\symbol{"F005}}}
\expandafter\def\csname faicon@star-o\endcsname{{\FA\symbol{"F006}}}
\expandafter\def\csname faicon@user\endcsname{{\FA\symbol{"F007}}}
\expandafter\def\csname faicon@film\endcsname{{\FA\symbol{"F008}}}
\expandafter\def\csname faicon@th-large\endcsname{{\FA\symbol{"F009}}}
\expandafter\def\csname faicon@th\endcsname{{\FA\symbol{"F00A}}}
\expandafter\def\csname faicon@th-list\endcsname{{\FA\symbol{"F00B}}}
\expandafter\def\csname faicon@check\endcsname{{\FA\symbol{"F00C}}}
\expandafter\def\csname faicon@times\endcsname{{\FA\symbol{"F00D}}}
\expandafter\def\csname faicon@search-plus\endcsname{{\FA\symbol{"F00E}}}
\expandafter\def\csname faicon@search-minus\endcsname{{\FA\symbol{"F010}}}
\expandafter\def\csname faicon@power-off\endcsname{{\FA\symbol{"F011}}}
\expandafter\def\csname faicon@signal\endcsname{{\FA\symbol{"F012}}}
\expandafter\def\csname faicon@cog\endcsname{{\FA\symbol{"F013}}}
\expandafter\def\csname faicon@trash-o\endcsname{{\FA\symbol{"F014}}}
\expandafter\def\csname faicon@home\endcsname{{\FA\symbol{"F015}}}
\expandafter\def\csname faicon@file-o\endcsname{{\FA\symbol{"F016}}}
\expandafter\def\csname faicon@clock-o\endcsname{{\FA\symbol{"F017}}}
\expandafter\def\csname faicon@road\endcsname{{\FA\symbol{"F018}}}
\expandafter\def\csname faicon@download\endcsname{{\FA\symbol{"F019}}}
\expandafter\def\csname faicon@arrow-circle-o-down\endcsname{{\FA\symbol{"F01A}}}
\expandafter\def\csname faicon@arrow-circle-o-up\endcsname{{\FA\symbol{"F01B}}}
\expandafter\def\csname faicon@inbox\endcsname{{\FA\symbol{"F01C}}}
\expandafter\def\csname faicon@play-circle-o\endcsname{{\FA\symbol{"F01D}}}
\expandafter\def\csname faicon@repeat\endcsname{{\FA\symbol{"F01E}}}
\expandafter\def\csname faicon@refresh\endcsname{{\FA\symbol{"F021}}}
\expandafter\def\csname faicon@list-alt\endcsname{{\FA\symbol{"F022}}}
\expandafter\def\csname faicon@lock\endcsname{{\FA\symbol{"F023}}}
\expandafter\def\csname faicon@flag\endcsname{{\FA\symbol{"F024}}}
\expandafter\def\csname faicon@headphones\endcsname{{\FA\symbol{"F025}}}
\expandafter\def\csname faicon@volume-off\endcsname{{\FA\symbol{"F026}}}
\expandafter\def\csname faicon@volume-down\endcsname{{\FA\symbol{"F027}}}
\expandafter\def\csname faicon@volume-up\endcsname{{\FA\symbol{"F028}}}
\expandafter\def\csname faicon@qrcode\endcsname{{\FA\symbol{"F029}}}
\expandafter\def\csname faicon@barcode\endcsname{{\FA\symbol{"F02A}}}
\expandafter\def\csname faicon@tag\endcsname{{\FA\symbol{"F02B}}}
\expandafter\def\csname faicon@tags\endcsname{{\FA\symbol{"F02C}}}
\expandafter\def\csname faicon@book\endcsname{{\FA\symbol{"F02D}}}
\expandafter\def\csname faicon@bookmark\endcsname{{\FA\symbol{"F02E}}}
\expandafter\def\csname faicon@print\endcsname{{\FA\symbol{"F02F}}}
\expandafter\def\csname faicon@camera\endcsname{{\FA\symbol{"F030}}}
\expandafter\def\csname faicon@font\endcsname{{\FA\symbol{"F031}}}
\expandafter\def\csname faicon@bold\endcsname{{\FA\symbol{"F032}}}
\expandafter\def\csname faicon@italic\endcsname{{\FA\symbol{"F033}}}
\expandafter\def\csname faicon@text-height\endcsname{{\FA\symbol{"F034}}}
\expandafter\def\csname faicon@text-width\endcsname{{\FA\symbol{"F035}}}
\expandafter\def\csname faicon@align-left\endcsname{{\FA\symbol{"F036}}}
\expandafter\def\csname faicon@align-center\endcsname{{\FA\symbol{"F037}}}
\expandafter\def\csname faicon@align-right\endcsname{{\FA\symbol{"F038}}}
\expandafter\def\csname faicon@align-justify\endcsname{{\FA\symbol{"F039}}}
\expandafter\def\csname faicon@list\endcsname{{\FA\symbol{"F03A}}}
\expandafter\def\csname faicon@outdent\endcsname{{\FA\symbol{"F03B}}}
\expandafter\def\csname faicon@indent\endcsname{{\FA\symbol{"F03C}}}
\expandafter\def\csname faicon@video-camera\endcsname{{\FA\symbol{"F03D}}}
\expandafter\def\csname faicon@picture-o\endcsname{{\FA\symbol{"F03E}}}
\expandafter\def\csname faicon@pencil\endcsname{{\FA\symbol{"F040}}}
\expandafter\def\csname faicon@map-marker\endcsname{{\FA\symbol{"F041}}}
\expandafter\def\csname faicon@adjust\endcsname{{\FA\symbol{"F042}}}
\expandafter\def\csname faicon@tint\endcsname{{\FA\symbol{"F043}}}
\expandafter\def\csname faicon@pencil-square-o\endcsname{{\FA\symbol{"F044}}}
\expandafter\def\csname faicon@share-square-o\endcsname{{\FA\symbol{"F045}}}
\expandafter\def\csname faicon@check-square-o\endcsname{{\FA\symbol{"F046}}}
\expandafter\def\csname faicon@arrows\endcsname{{\FA\symbol{"F047}}}
\expandafter\def\csname faicon@step-backward\endcsname{{\FA\symbol{"F048}}}
\expandafter\def\csname faicon@fast-backward\endcsname{{\FA\symbol{"F049}}}
\expandafter\def\csname faicon@backward\endcsname{{\FA\symbol{"F04A}}}
\expandafter\def\csname faicon@play\endcsname{{\FA\symbol{"F04B}}}
\expandafter\def\csname faicon@pause\endcsname{{\FA\symbol{"F04C}}}
\expandafter\def\csname faicon@stop\endcsname{{\FA\symbol{"F04D}}}
\expandafter\def\csname faicon@forward\endcsname{{\FA\symbol{"F04E}}}
\expandafter\def\csname faicon@fast-forward\endcsname{{\FA\symbol{"F050}}}
\expandafter\def\csname faicon@step-forward\endcsname{{\FA\symbol{"F051}}}
\expandafter\def\csname faicon@eject\endcsname{{\FA\symbol{"F052}}}
\expandafter\def\csname faicon@chevron-left\endcsname{{\FA\symbol{"F053}}}
\expandafter\def\csname faicon@chevron-right\endcsname{{\FA\symbol{"F054}}}
\expandafter\def\csname faicon@plus-circle\endcsname{{\FA\symbol{"F055}}}
\expandafter\def\csname faicon@minus-circle\endcsname{{\FA\symbol{"F056}}}
\expandafter\def\csname faicon@times-circle\endcsname{{\FA\symbol{"F057}}}
\expandafter\def\csname faicon@check-circle\endcsname{{\FA\symbol{"F058}}}
\expandafter\def\csname faicon@question-circle\endcsname{{\FA\symbol{"F059}}}
\expandafter\def\csname faicon@info-circle\endcsname{{\FA\symbol{"F05A}}}
\expandafter\def\csname faicon@crosshairs\endcsname{{\FA\symbol{"F05B}}}
\expandafter\def\csname faicon@times-circle-o\endcsname{{\FA\symbol{"F05C}}}
\expandafter\def\csname faicon@check-circle-o\endcsname{{\FA\symbol{"F05D}}}
\expandafter\def\csname faicon@ban\endcsname{{\FA\symbol{"F05E}}}
\expandafter\def\csname faicon@arrow-left\endcsname{{\FA\symbol{"F060}}}
\expandafter\def\csname faicon@arrow-right\endcsname{{\FA\symbol{"F061}}}
\expandafter\def\csname faicon@arrow-up\endcsname{{\FA\symbol{"F062}}}
\expandafter\def\csname faicon@arrow-down\endcsname{{\FA\symbol{"F063}}}
\expandafter\def\csname faicon@share\endcsname{{\FA\symbol{"F064}}}
\expandafter\def\csname faicon@expand\endcsname{{\FA\symbol{"F065}}}
\expandafter\def\csname faicon@compress\endcsname{{\FA\symbol{"F066}}}
\expandafter\def\csname faicon@plus\endcsname{{\FA\symbol{"F067}}}
\expandafter\def\csname faicon@minus\endcsname{{\FA\symbol{"F068}}}
\expandafter\def\csname faicon@asterisk\endcsname{{\FA\symbol{"F069}}}
\expandafter\def\csname faicon@exclamation-circle\endcsname{{\FA\symbol{"F06A}}}
\expandafter\def\csname faicon@gift\endcsname{{\FA\symbol{"F06B}}}
\expandafter\def\csname faicon@leaf\endcsname{{\FA\symbol{"F06C}}}
\expandafter\def\csname faicon@fire\endcsname{{\FA\symbol{"F06D}}}
\expandafter\def\csname faicon@eye\endcsname{{\FA\symbol{"F06E}}}
\expandafter\def\csname faicon@eye-slash\endcsname{{\FA\symbol{"F070}}}
\expandafter\def\csname faicon@exclamation-triangle\endcsname{{\FA\symbol{"F071}}}
\expandafter\def\csname faicon@plane\endcsname{{\FA\symbol{"F072}}}
\expandafter\def\csname faicon@calendar\endcsname{{\FA\symbol{"F073}}}
\expandafter\def\csname faicon@random\endcsname{{\FA\symbol{"F074}}}
\expandafter\def\csname faicon@comment\endcsname{{\FA\symbol{"F075}}}
\expandafter\def\csname faicon@magnet\endcsname{{\FA\symbol{"F076}}}
\expandafter\def\csname faicon@chevron-up\endcsname{{\FA\symbol{"F077}}}
\expandafter\def\csname faicon@chevron-down\endcsname{{\FA\symbol{"F078}}}
\expandafter\def\csname faicon@retweet\endcsname{{\FA\symbol{"F079}}}
\expandafter\def\csname faicon@shopping-cart\endcsname{{\FA\symbol{"F07A}}}
\expandafter\def\csname faicon@folder\endcsname{{\FA\symbol{"F07B}}}
\expandafter\def\csname faicon@folder-open\endcsname{{\FA\symbol{"F07C}}}
\expandafter\def\csname faicon@arrows-v\endcsname{{\FA\symbol{"F07D}}}
\expandafter\def\csname faicon@arrows-h\endcsname{{\FA\symbol{"F07E}}}
\expandafter\def\csname faicon@bar-chart\endcsname{{\FA\symbol{"F080}}}
\expandafter\def\csname faicon@twitter-square\endcsname{{\FA\symbol{"F081}}}
\expandafter\def\csname faicon@facebook-square\endcsname{{\FA\symbol{"F082}}}
\expandafter\def\csname faicon@camera-retro\endcsname{{\FA\symbol{"F083}}}
\expandafter\def\csname faicon@key\endcsname{{\FA\symbol{"F084}}}
\expandafter\def\csname faicon@cogs\endcsname{{\FA\symbol{"F085}}}
\expandafter\def\csname faicon@comments\endcsname{{\FA\symbol{"F086}}}
\expandafter\def\csname faicon@thumbs-o-up\endcsname{{\FA\symbol{"F087}}}
\expandafter\def\csname faicon@thumbs-o-down\endcsname{{\FA\symbol{"F088}}}
\expandafter\def\csname faicon@star-half\endcsname{{\FA\symbol{"F089}}}
\expandafter\def\csname faicon@heart-o\endcsname{{\FA\symbol{"F08A}}}
\expandafter\def\csname faicon@sign-out\endcsname{{\FA\symbol{"F08B}}}
\expandafter\def\csname faicon@linkedin-square\endcsname{{\FA\symbol{"F08C}}}
\expandafter\def\csname faicon@thumb-tack\endcsname{{\FA\symbol{"F08D}}}
\expandafter\def\csname faicon@external-link\endcsname{{\FA\symbol{"F08E}}}
\expandafter\def\csname faicon@sign-in\endcsname{{\FA\symbol{"F090}}}
\expandafter\def\csname faicon@trophy\endcsname{{\FA\symbol{"F091}}}
\expandafter\def\csname faicon@github-square\endcsname{{\FA\symbol{"F092}}}
\expandafter\def\csname faicon@upload\endcsname{{\FA\symbol{"F093}}}
\expandafter\def\csname faicon@lemon-o\endcsname{{\FA\symbol{"F094}}}
\expandafter\def\csname faicon@phone\endcsname{{\FA\symbol{"F095}}}
\expandafter\def\csname faicon@square-o\endcsname{{\FA\symbol{"F096}}}
\expandafter\def\csname faicon@bookmark-o\endcsname{{\FA\symbol{"F097}}}
\expandafter\def\csname faicon@phone-square\endcsname{{\FA\symbol{"F098}}}
\expandafter\def\csname faicon@twitter\endcsname{{\FA\symbol{"F099}}}
\expandafter\def\csname faicon@facebook\endcsname{{\FA\symbol{"F09A}}}
\expandafter\def\csname faicon@github\endcsname{{\FA\symbol{"F09B}}}
\expandafter\def\csname faicon@unlock\endcsname{{\FA\symbol{"F09C}}}
\expandafter\def\csname faicon@credit-card\endcsname{{\FA\symbol{"F09D}}}
\expandafter\def\csname faicon@rss\endcsname{{\FA\symbol{"F09E}}}
\expandafter\def\csname faicon@hdd-o\endcsname{{\FA\symbol{"F0A0}}}
\expandafter\def\csname faicon@bullhorn\endcsname{{\FA\symbol{"F0A1}}}
\expandafter\def\csname faicon@bell\endcsname{{\FA\symbol{"F0F3}}}
\expandafter\def\csname faicon@certificate\endcsname{{\FA\symbol{"F0A3}}}
\expandafter\def\csname faicon@hand-o-right\endcsname{{\FA\symbol{"F0A4}}}
\expandafter\def\csname faicon@hand-o-left\endcsname{{\FA\symbol{"F0A5}}}
\expandafter\def\csname faicon@hand-o-up\endcsname{{\FA\symbol{"F0A6}}}
\expandafter\def\csname faicon@hand-o-down\endcsname{{\FA\symbol{"F0A7}}}
\expandafter\def\csname faicon@arrow-circle-left\endcsname{{\FA\symbol{"F0A8}}}
\expandafter\def\csname faicon@arrow-circle-right\endcsname{{\FA\symbol{"F0A9}}}
\expandafter\def\csname faicon@arrow-circle-up\endcsname{{\FA\symbol{"F0AA}}}
\expandafter\def\csname faicon@arrow-circle-down\endcsname{{\FA\symbol{"F0AB}}}
\expandafter\def\csname faicon@globe\endcsname{{\FA\symbol{"F0AC}}}
\expandafter\def\csname faicon@wrench\endcsname{{\FA\symbol{"F0AD}}}
\expandafter\def\csname faicon@tasks\endcsname{{\FA\symbol{"F0AE}}}
\expandafter\def\csname faicon@filter\endcsname{{\FA\symbol{"F0B0}}}
\expandafter\def\csname faicon@briefcase\endcsname{{\FA\symbol{"F0B1}}}
\expandafter\def\csname faicon@arrows-alt\endcsname{{\FA\symbol{"F0B2}}}
\expandafter\def\csname faicon@users\endcsname{{\FA\symbol{"F0C0}}}
\expandafter\def\csname faicon@link\endcsname{{\FA\symbol{"F0C1}}}
\expandafter\def\csname faicon@cloud\endcsname{{\FA\symbol{"F0C2}}}
\expandafter\def\csname faicon@flask\endcsname{{\FA\symbol{"F0C3}}}
\expandafter\def\csname faicon@scissors\endcsname{{\FA\symbol{"F0C4}}}
\expandafter\def\csname faicon@files-o\endcsname{{\FA\symbol{"F0C5}}}
\expandafter\def\csname faicon@paperclip\endcsname{{\FA\symbol{"F0C6}}}
\expandafter\def\csname faicon@floppy-o\endcsname{{\FA\symbol{"F0C7}}}
\expandafter\def\csname faicon@square\endcsname{{\FA\symbol{"F0C8}}}
\expandafter\def\csname faicon@bars\endcsname{{\FA\symbol{"F0C9}}}
\expandafter\def\csname faicon@list-ul\endcsname{{\FA\symbol{"F0CA}}}
\expandafter\def\csname faicon@list-ol\endcsname{{\FA\symbol{"F0CB}}}
\expandafter\def\csname faicon@strikethrough\endcsname{{\FA\symbol{"F0CC}}}
\expandafter\def\csname faicon@underline\endcsname{{\FA\symbol{"F0CD}}}
\expandafter\def\csname faicon@table\endcsname{{\FA\symbol{"F0CE}}}
\expandafter\def\csname faicon@magic\endcsname{{\FA\symbol{"F0D0}}}
\expandafter\def\csname faicon@truck\endcsname{{\FA\symbol{"F0D1}}}
\expandafter\def\csname faicon@pinterest\endcsname{{\FA\symbol{"F0D2}}}
\expandafter\def\csname faicon@pinterest-square\endcsname{{\FA\symbol{"F0D3}}}
\expandafter\def\csname faicon@google-plus-square\endcsname{{\FA\symbol{"F0D4}}}
\expandafter\def\csname faicon@google-plus\endcsname{{\FA\symbol{"F0D5}}}
\expandafter\def\csname faicon@money\endcsname{{\FA\symbol{"F0D6}}}
\expandafter\def\csname faicon@caret-down\endcsname{{\FA\symbol{"F0D7}}}
\expandafter\def\csname faicon@caret-up\endcsname{{\FA\symbol{"F0D8}}}
\expandafter\def\csname faicon@caret-left\endcsname{{\FA\symbol{"F0D9}}}
\expandafter\def\csname faicon@caret-right\endcsname{{\FA\symbol{"F0DA}}}
\expandafter\def\csname faicon@columns\endcsname{{\FA\symbol{"F0DB}}}
\expandafter\def\csname faicon@sort\endcsname{{\FA\symbol{"F0DC}}}
\expandafter\def\csname faicon@sort-desc\endcsname{{\FA\symbol{"F0DD}}}
\expandafter\def\csname faicon@sort-asc\endcsname{{\FA\symbol{"F0DE}}}
\expandafter\def\csname faicon@envelope\endcsname{{\FA\symbol{"F0E0}}}
\expandafter\def\csname faicon@linkedin\endcsname{{\FA\symbol{"F0E1}}}
\expandafter\def\csname faicon@undo\endcsname{{\FA\symbol{"F0E2}}}
\expandafter\def\csname faicon@gavel\endcsname{{\FA\symbol{"F0E3}}}
\expandafter\def\csname faicon@tachometer\endcsname{{\FA\symbol{"F0E4}}}
\expandafter\def\csname faicon@comment-o\endcsname{{\FA\symbol{"F0E5}}}
\expandafter\def\csname faicon@comments-o\endcsname{{\FA\symbol{"F0E6}}}
\expandafter\def\csname faicon@bolt\endcsname{{\FA\symbol{"F0E7}}}
\expandafter\def\csname faicon@sitemap\endcsname{{\FA\symbol{"F0E8}}}
\expandafter\def\csname faicon@umbrella\endcsname{{\FA\symbol{"F0E9}}}
\expandafter\def\csname faicon@clipboard\endcsname{{\FA\symbol{"F0EA}}}
\expandafter\def\csname faicon@lightbulb-o\endcsname{{\FA\symbol{"F0EB}}}
\expandafter\def\csname faicon@exchange\endcsname{{\FA\symbol{"F0EC}}}
\expandafter\def\csname faicon@cloud-download\endcsname{{\FA\symbol{"F0ED}}}
\expandafter\def\csname faicon@cloud-upload\endcsname{{\FA\symbol{"F0EE}}}
\expandafter\def\csname faicon@user-md\endcsname{{\FA\symbol{"F0F0}}}
\expandafter\def\csname faicon@stethoscope\endcsname{{\FA\symbol{"F0F1}}}
\expandafter\def\csname faicon@suitcase\endcsname{{\FA\symbol{"F0F2}}}
\expandafter\def\csname faicon@bell-o\endcsname{{\FA\symbol{"F0A2}}}
\expandafter\def\csname faicon@coffee\endcsname{{\FA\symbol{"F0F4}}}
\expandafter\def\csname faicon@cutlery\endcsname{{\FA\symbol{"F0F5}}}
\expandafter\def\csname faicon@file-text-o\endcsname{{\FA\symbol{"F0F6}}}
\expandafter\def\csname faicon@building-o\endcsname{{\FA\symbol{"F0F7}}}
\expandafter\def\csname faicon@hospital-o\endcsname{{\FA\symbol{"F0F8}}}
\expandafter\def\csname faicon@ambulance\endcsname{{\FA\symbol{"F0F9}}}
\expandafter\def\csname faicon@medkit\endcsname{{\FA\symbol{"F0FA}}}
\expandafter\def\csname faicon@fighter-jet\endcsname{{\FA\symbol{"F0FB}}}
\expandafter\def\csname faicon@beer\endcsname{{\FA\symbol{"F0FC}}}
\expandafter\def\csname faicon@h-square\endcsname{{\FA\symbol{"F0FD}}}
\expandafter\def\csname faicon@plus-square\endcsname{{\FA\symbol{"F0FE}}}
\expandafter\def\csname faicon@angle-double-left\endcsname{{\FA\symbol{"F100}}}
\expandafter\def\csname faicon@angle-double-right\endcsname{{\FA\symbol{"F101}}}
\expandafter\def\csname faicon@angle-double-up\endcsname{{\FA\symbol{"F102}}}
\expandafter\def\csname faicon@angle-double-down\endcsname{{\FA\symbol{"F103}}}
\expandafter\def\csname faicon@angle-left\endcsname{{\FA\symbol{"F104}}}
\expandafter\def\csname faicon@angle-right\endcsname{{\FA\symbol{"F105}}}
\expandafter\def\csname faicon@angle-up\endcsname{{\FA\symbol{"F106}}}
\expandafter\def\csname faicon@angle-down\endcsname{{\FA\symbol{"F107}}}
\expandafter\def\csname faicon@desktop\endcsname{{\FA\symbol{"F108}}}
\expandafter\def\csname faicon@laptop\endcsname{{\FA\symbol{"F109}}}
\expandafter\def\csname faicon@tablet\endcsname{{\FA\symbol{"F10A}}}
\expandafter\def\csname faicon@mobile\endcsname{{\FA\symbol{"F10B}}}
\expandafter\def\csname faicon@circle-o\endcsname{{\FA\symbol{"F10C}}}
\expandafter\def\csname faicon@quote-left\endcsname{{\FA\symbol{"F10D}}}
\expandafter\def\csname faicon@quote-right\endcsname{{\FA\symbol{"F10E}}}
\expandafter\def\csname faicon@spinner\endcsname{{\FA\symbol{"F110}}}
\expandafter\def\csname faicon@circle\endcsname{{\FA\symbol{"F111}}}
\expandafter\def\csname faicon@reply\endcsname{{\FA\symbol{"F112}}}
\expandafter\def\csname faicon@github-alt\endcsname{{\FA\symbol{"F113}}}
\expandafter\def\csname faicon@folder-o\endcsname{{\FA\symbol{"F114}}}
\expandafter\def\csname faicon@folder-open-o\endcsname{{\FA\symbol{"F115}}}
\expandafter\def\csname faicon@smile-o\endcsname{{\FA\symbol{"F118}}}
\expandafter\def\csname faicon@frown-o\endcsname{{\FA\symbol{"F119}}}
\expandafter\def\csname faicon@meh-o\endcsname{{\FA\symbol{"F11A}}}
\expandafter\def\csname faicon@gamepad\endcsname{{\FA\symbol{"F11B}}}
\expandafter\def\csname faicon@keyboard-o\endcsname{{\FA\symbol{"F11C}}}
\expandafter\def\csname faicon@flag-o\endcsname{{\FA\symbol{"F11D}}}
\expandafter\def\csname faicon@flag-checkered\endcsname{{\FA\symbol{"F11E}}}
\expandafter\def\csname faicon@terminal\endcsname{{\FA\symbol{"F120}}}
\expandafter\def\csname faicon@code\endcsname{{\FA\symbol{"F121}}}
\expandafter\def\csname faicon@reply-all\endcsname{{\FA\symbol{"F122}}}
\expandafter\def\csname faicon@star-half-o\endcsname{{\FA\symbol{"F123}}}
\expandafter\def\csname faicon@location-arrow\endcsname{{\FA\symbol{"F124}}}
\expandafter\def\csname faicon@crop\endcsname{{\FA\symbol{"F125}}}
\expandafter\def\csname faicon@code-fork\endcsname{{\FA\symbol{"F126}}}
\expandafter\def\csname faicon@chain-broken\endcsname{{\FA\symbol{"F127}}}
\expandafter\def\csname faicon@question\endcsname{{\FA\symbol{"F128}}}
\expandafter\def\csname faicon@info\endcsname{{\FA\symbol{"F129}}}
\expandafter\def\csname faicon@exclamation\endcsname{{\FA\symbol{"F12A}}}
\expandafter\def\csname faicon@superscript\endcsname{{\FA\symbol{"F12B}}}
\expandafter\def\csname faicon@subscript\endcsname{{\FA\symbol{"F12C}}}
\expandafter\def\csname faicon@eraser\endcsname{{\FA\symbol{"F12D}}}
\expandafter\def\csname faicon@puzzle-piece\endcsname{{\FA\symbol{"F12E}}}
\expandafter\def\csname faicon@microphone\endcsname{{\FA\symbol{"F130}}}
\expandafter\def\csname faicon@microphone-slash\endcsname{{\FA\symbol{"F131}}}
\expandafter\def\csname faicon@shield\endcsname{{\FA\symbol{"F132}}}
\expandafter\def\csname faicon@calendar-o\endcsname{{\FA\symbol{"F133}}}
\expandafter\def\csname faicon@fire-extinguisher\endcsname{{\FA\symbol{"F134}}}
\expandafter\def\csname faicon@rocket\endcsname{{\FA\symbol{"F135}}}
\expandafter\def\csname faicon@maxcdn\endcsname{{\FA\symbol{"F136}}}
\expandafter\def\csname faicon@chevron-circle-left\endcsname{{\FA\symbol{"F137}}}
\expandafter\def\csname faicon@chevron-circle-right\endcsname{{\FA\symbol{"F138}}}
\expandafter\def\csname faicon@chevron-circle-up\endcsname{{\FA\symbol{"F139}}}
\expandafter\def\csname faicon@chevron-circle-down\endcsname{{\FA\symbol{"F13A}}}
\expandafter\def\csname faicon@html5\endcsname{{\FA\symbol{"F13B}}}
\expandafter\def\csname faicon@css3\endcsname{{\FA\symbol{"F13C}}}
\expandafter\def\csname faicon@anchor\endcsname{{\FA\symbol{"F13D}}}
\expandafter\def\csname faicon@unlock-alt\endcsname{{\FA\symbol{"F13E}}}
\expandafter\def\csname faicon@bullseye\endcsname{{\FA\symbol{"F140}}}
\expandafter\def\csname faicon@ellipsis-h\endcsname{{\FA\symbol{"F141}}}
\expandafter\def\csname faicon@ellipsis-v\endcsname{{\FA\symbol{"F142}}}
\expandafter\def\csname faicon@rss-square\endcsname{{\FA\symbol{"F143}}}
\expandafter\def\csname faicon@play-circle\endcsname{{\FA\symbol{"F144}}}
\expandafter\def\csname faicon@ticket\endcsname{{\FA\symbol{"F145}}}
\expandafter\def\csname faicon@minus-square\endcsname{{\FA\symbol{"F146}}}
\expandafter\def\csname faicon@minus-square-o\endcsname{{\FA\symbol{"F147}}}
\expandafter\def\csname faicon@level-up\endcsname{{\FA\symbol{"F148}}}
\expandafter\def\csname faicon@level-down\endcsname{{\FA\symbol{"F149}}}
\expandafter\def\csname faicon@check-square\endcsname{{\FA\symbol{"F14A}}}
\expandafter\def\csname faicon@pencil-square\endcsname{{\FA\symbol{"F14B}}}
\expandafter\def\csname faicon@external-link-square\endcsname{{\FA\symbol{"F14C}}}
\expandafter\def\csname faicon@share-square\endcsname{{\FA\symbol{"F14D}}}
\expandafter\def\csname faicon@compass\endcsname{{\FA\symbol{"F14E}}}
\expandafter\def\csname faicon@caret-square-o-down\endcsname{{\FA\symbol{"F150}}}
\expandafter\def\csname faicon@caret-square-o-up\endcsname{{\FA\symbol{"F151}}}
\expandafter\def\csname faicon@caret-square-o-right\endcsname{{\FA\symbol{"F152}}}
\expandafter\def\csname faicon@eur\endcsname{{\FA\symbol{"F153}}}
\expandafter\def\csname faicon@gbp\endcsname{{\FA\symbol{"F154}}}
\expandafter\def\csname faicon@usd\endcsname{{\FA\symbol{"F155}}}
\expandafter\def\csname faicon@inr\endcsname{{\FA\symbol{"F156}}}
\expandafter\def\csname faicon@jpy\endcsname{{\FA\symbol{"F157}}}
\expandafter\def\csname faicon@rub\endcsname{{\FA\symbol{"F158}}}
\expandafter\def\csname faicon@krw\endcsname{{\FA\symbol{"F159}}}
\expandafter\def\csname faicon@btc\endcsname{{\FA\symbol{"F15A}}}
\expandafter\def\csname faicon@file\endcsname{{\FA\symbol{"F15B}}}
\expandafter\def\csname faicon@file-text\endcsname{{\FA\symbol{"F15C}}}
\expandafter\def\csname faicon@sort-alpha-asc\endcsname{{\FA\symbol{"F15D}}}
\expandafter\def\csname faicon@sort-alpha-desc\endcsname{{\FA\symbol{"F15E}}}
\expandafter\def\csname faicon@sort-amount-asc\endcsname{{\FA\symbol{"F160}}}
\expandafter\def\csname faicon@sort-amount-desc\endcsname{{\FA\symbol{"F161}}}
\expandafter\def\csname faicon@sort-numeric-asc\endcsname{{\FA\symbol{"F162}}}
\expandafter\def\csname faicon@sort-numeric-desc\endcsname{{\FA\symbol{"F163}}}
\expandafter\def\csname faicon@thumbs-up\endcsname{{\FA\symbol{"F164}}}
\expandafter\def\csname faicon@thumbs-down\endcsname{{\FA\symbol{"F165}}}
\expandafter\def\csname faicon@youtube-square\endcsname{{\FA\symbol{"F166}}}
\expandafter\def\csname faicon@youtube\endcsname{{\FA\symbol{"F167}}}
\expandafter\def\csname faicon@xing\endcsname{{\FA\symbol{"F168}}}
\expandafter\def\csname faicon@xing-square\endcsname{{\FA\symbol{"F169}}}
\expandafter\def\csname faicon@youtube-play\endcsname{{\FA\symbol{"F16A}}}
\expandafter\def\csname faicon@dropbox\endcsname{{\FA\symbol{"F16B}}}
\expandafter\def\csname faicon@stack-overflow\endcsname{{\FA\symbol{"F16C}}}
\expandafter\def\csname faicon@instagram\endcsname{{\FA\symbol{"F16D}}}
\expandafter\def\csname faicon@flickr\endcsname{{\FA\symbol{"F16E}}}
\expandafter\def\csname faicon@adn\endcsname{{\FA\symbol{"F170}}}
\expandafter\def\csname faicon@bitbucket\endcsname{{\FA\symbol{"F171}}}
\expandafter\def\csname faicon@bitbucket-square\endcsname{{\FA\symbol{"F172}}}
\expandafter\def\csname faicon@tumblr\endcsname{{\FA\symbol{"F173}}}
\expandafter\def\csname faicon@tumblr-square\endcsname{{\FA\symbol{"F174}}}
\expandafter\def\csname faicon@long-arrow-down\endcsname{{\FA\symbol{"F175}}}
\expandafter\def\csname faicon@long-arrow-up\endcsname{{\FA\symbol{"F176}}}
\expandafter\def\csname faicon@long-arrow-left\endcsname{{\FA\symbol{"F177}}}
\expandafter\def\csname faicon@long-arrow-right\endcsname{{\FA\symbol{"F178}}}
\expandafter\def\csname faicon@apple\endcsname{{\FA\symbol{"F179}}}
\expandafter\def\csname faicon@windows\endcsname{{\FA\symbol{"F17A}}}
\expandafter\def\csname faicon@android\endcsname{{\FA\symbol{"F17B}}}
\expandafter\def\csname faicon@linux\endcsname{{\FA\symbol{"F17C}}}
\expandafter\def\csname faicon@dribbble\endcsname{{\FA\symbol{"F17D}}}
\expandafter\def\csname faicon@skype\endcsname{{\FA\symbol{"F17E}}}
\expandafter\def\csname faicon@foursquare\endcsname{{\FA\symbol{"F180}}}
\expandafter\def\csname faicon@trello\endcsname{{\FA\symbol{"F181}}}
\expandafter\def\csname faicon@female\endcsname{{\FA\symbol{"F182}}}
\expandafter\def\csname faicon@male\endcsname{{\FA\symbol{"F183}}}
\expandafter\def\csname faicon@gratipay\endcsname{{\FA\symbol{"F184}}}
\expandafter\def\csname faicon@sun-o\endcsname{{\FA\symbol{"F185}}}
\expandafter\def\csname faicon@moon-o\endcsname{{\FA\symbol{"F186}}}
\expandafter\def\csname faicon@archive\endcsname{{\FA\symbol{"F187}}}
\expandafter\def\csname faicon@bug\endcsname{{\FA\symbol{"F188}}}
\expandafter\def\csname faicon@vk\endcsname{{\FA\symbol{"F189}}}
\expandafter\def\csname faicon@weibo\endcsname{{\FA\symbol{"F18A}}}
\expandafter\def\csname faicon@renren\endcsname{{\FA\symbol{"F18B}}}
\expandafter\def\csname faicon@pagelines\endcsname{{\FA\symbol{"F18C}}}
\expandafter\def\csname faicon@stack-exchange\endcsname{{\FA\symbol{"F18D}}}
\expandafter\def\csname faicon@arrow-circle-o-right\endcsname{{\FA\symbol{"F18E}}}
\expandafter\def\csname faicon@arrow-circle-o-left\endcsname{{\FA\symbol{"F190}}}
\expandafter\def\csname faicon@caret-square-o-left\endcsname{{\FA\symbol{"F191}}}
\expandafter\def\csname faicon@dot-circle-o\endcsname{{\FA\symbol{"F192}}}
\expandafter\def\csname faicon@wheelchair\endcsname{{\FA\symbol{"F193}}}
\expandafter\def\csname faicon@vimeo-square\endcsname{{\FA\symbol{"F194}}}
\expandafter\def\csname faicon@try\endcsname{{\FA\symbol{"F195}}}
\expandafter\def\csname faicon@plus-square-o\endcsname{{\FA\symbol{"F196}}}
\expandafter\def\csname faicon@space-shuttle\endcsname{{\FA\symbol{"F197}}}
\expandafter\def\csname faicon@slack\endcsname{{\FA\symbol{"F198}}}
\expandafter\def\csname faicon@envelope-square\endcsname{{\FA\symbol{"F199}}}
\expandafter\def\csname faicon@wordpress\endcsname{{\FA\symbol{"F19A}}}
\expandafter\def\csname faicon@openid\endcsname{{\FA\symbol{"F19B}}}
\expandafter\def\csname faicon@university\endcsname{{\FA\symbol{"F19C}}}
\expandafter\def\csname faicon@graduation-cap\endcsname{{\FA\symbol{"F19D}}}
\expandafter\def\csname faicon@yahoo\endcsname{{\FA\symbol{"F19E}}}
\expandafter\def\csname faicon@google\endcsname{{\FA\symbol{"F1A0}}}
\expandafter\def\csname faicon@reddit\endcsname{{\FA\symbol{"F1A1}}}
\expandafter\def\csname faicon@reddit-square\endcsname{{\FA\symbol{"F1A2}}}
\expandafter\def\csname faicon@stumbleupon-circle\endcsname{{\FA\symbol{"F1A3}}}
\expandafter\def\csname faicon@stumbleupon\endcsname{{\FA\symbol{"F1A4}}}
\expandafter\def\csname faicon@delicious\endcsname{{\FA\symbol{"F1A5}}}
\expandafter\def\csname faicon@digg\endcsname{{\FA\symbol{"F1A6}}}
\expandafter\def\csname faicon@pied-piper-pp\endcsname{{\FA\symbol{"F1A7}}}
\expandafter\def\csname faicon@pied-piper-alt\endcsname{{\FA\symbol{"F1A8}}}
\expandafter\def\csname faicon@drupal\endcsname{{\FA\symbol{"F1A9}}}
\expandafter\def\csname faicon@joomla\endcsname{{\FA\symbol{"F1AA}}}
\expandafter\def\csname faicon@language\endcsname{{\FA\symbol{"F1AB}}}
\expandafter\def\csname faicon@fax\endcsname{{\FA\symbol{"F1AC}}}
\expandafter\def\csname faicon@building\endcsname{{\FA\symbol{"F1AD}}}
\expandafter\def\csname faicon@child\endcsname{{\FA\symbol{"F1AE}}}
\expandafter\def\csname faicon@paw\endcsname{{\FA\symbol{"F1B0}}}
\expandafter\def\csname faicon@spoon\endcsname{{\FA\symbol{"F1B1}}}
\expandafter\def\csname faicon@cube\endcsname{{\FA\symbol{"F1B2}}}
\expandafter\def\csname faicon@cubes\endcsname{{\FA\symbol{"F1B3}}}
\expandafter\def\csname faicon@behance\endcsname{{\FA\symbol{"F1B4}}}
\expandafter\def\csname faicon@behance-square\endcsname{{\FA\symbol{"F1B5}}}
\expandafter\def\csname faicon@steam\endcsname{{\FA\symbol{"F1B6}}}
\expandafter\def\csname faicon@steam-square\endcsname{{\FA\symbol{"F1B7}}}
\expandafter\def\csname faicon@recycle\endcsname{{\FA\symbol{"F1B8}}}
\expandafter\def\csname faicon@car\endcsname{{\FA\symbol{"F1B9}}}
\expandafter\def\csname faicon@taxi\endcsname{{\FA\symbol{"F1BA}}}
\expandafter\def\csname faicon@tree\endcsname{{\FA\symbol{"F1BB}}}
\expandafter\def\csname faicon@spotify\endcsname{{\FA\symbol{"F1BC}}}
\expandafter\def\csname faicon@deviantart\endcsname{{\FA\symbol{"F1BD}}}
\expandafter\def\csname faicon@soundcloud\endcsname{{\FA\symbol{"F1BE}}}
\expandafter\def\csname faicon@database\endcsname{{\FA\symbol{"F1C0}}}
\expandafter\def\csname faicon@file-pdf-o\endcsname{{\FA\symbol{"F1C1}}}
\expandafter\def\csname faicon@file-word-o\endcsname{{\FA\symbol{"F1C2}}}
\expandafter\def\csname faicon@file-excel-o\endcsname{{\FA\symbol{"F1C3}}}
\expandafter\def\csname faicon@file-powerpoint-o\endcsname{{\FA\symbol{"F1C4}}}
\expandafter\def\csname faicon@file-image-o\endcsname{{\FA\symbol{"F1C5}}}
\expandafter\def\csname faicon@file-archive-o\endcsname{{\FA\symbol{"F1C6}}}
\expandafter\def\csname faicon@file-audio-o\endcsname{{\FA\symbol{"F1C7}}}
\expandafter\def\csname faicon@file-video-o\endcsname{{\FA\symbol{"F1C8}}}
\expandafter\def\csname faicon@file-code-o\endcsname{{\FA\symbol{"F1C9}}}
\expandafter\def\csname faicon@vine\endcsname{{\FA\symbol{"F1CA}}}
\expandafter\def\csname faicon@codepen\endcsname{{\FA\symbol{"F1CB}}}
\expandafter\def\csname faicon@jsfiddle\endcsname{{\FA\symbol{"F1CC}}}
\expandafter\def\csname faicon@life-ring\endcsname{{\FA\symbol{"F1CD}}}
\expandafter\def\csname faicon@circle-o-notch\endcsname{{\FA\symbol{"F1CE}}}
\expandafter\def\csname faicon@rebel\endcsname{{\FA\symbol{"F1D0}}}
\expandafter\def\csname faicon@empire\endcsname{{\FA\symbol{"F1D1}}}
\expandafter\def\csname faicon@git-square\endcsname{{\FA\symbol{"F1D2}}}
\expandafter\def\csname faicon@git\endcsname{{\FA\symbol{"F1D3}}}
\expandafter\def\csname faicon@hacker-news\endcsname{{\FA\symbol{"F1D4}}}
\expandafter\def\csname faicon@tencent-weibo\endcsname{{\FA\symbol{"F1D5}}}
\expandafter\def\csname faicon@qq\endcsname{{\FA\symbol{"F1D6}}}
\expandafter\def\csname faicon@weixin\endcsname{{\FA\symbol{"F1D7}}}
\expandafter\def\csname faicon@paper-plane\endcsname{{\FA\symbol{"F1D8}}}
\expandafter\def\csname faicon@paper-plane-o\endcsname{{\FA\symbol{"F1D9}}}
\expandafter\def\csname faicon@history\endcsname{{\FA\symbol{"F1DA}}}
\expandafter\def\csname faicon@circle-thin\endcsname{{\FA\symbol{"F1DB}}}
\expandafter\def\csname faicon@header\endcsname{{\FA\symbol{"F1DC}}}
\expandafter\def\csname faicon@paragraph\endcsname{{\FA\symbol{"F1DD}}}
\expandafter\def\csname faicon@sliders\endcsname{{\FA\symbol{"F1DE}}}
\expandafter\def\csname faicon@share-alt\endcsname{{\FA\symbol{"F1E0}}}
\expandafter\def\csname faicon@share-alt-square\endcsname{{\FA\symbol{"F1E1}}}
\expandafter\def\csname faicon@bomb\endcsname{{\FA\symbol{"F1E2}}}
\expandafter\def\csname faicon@futbol-o\endcsname{{\FA\symbol{"F1E3}}}
\expandafter\def\csname faicon@tty\endcsname{{\FA\symbol{"F1E4}}}
\expandafter\def\csname faicon@binoculars\endcsname{{\FA\symbol{"F1E5}}}
\expandafter\def\csname faicon@plug\endcsname{{\FA\symbol{"F1E6}}}
\expandafter\def\csname faicon@slideshare\endcsname{{\FA\symbol{"F1E7}}}
\expandafter\def\csname faicon@twitch\endcsname{{\FA\symbol{"F1E8}}}
\expandafter\def\csname faicon@yelp\endcsname{{\FA\symbol{"F1E9}}}
\expandafter\def\csname faicon@newspaper-o\endcsname{{\FA\symbol{"F1EA}}}
\expandafter\def\csname faicon@wifi\endcsname{{\FA\symbol{"F1EB}}}
\expandafter\def\csname faicon@calculator\endcsname{{\FA\symbol{"F1EC}}}
\expandafter\def\csname faicon@paypal\endcsname{{\FA\symbol{"F1ED}}}
\expandafter\def\csname faicon@google-wallet\endcsname{{\FA\symbol{"F1EE}}}
\expandafter\def\csname faicon@cc-visa\endcsname{{\FA\symbol{"F1F0}}}
\expandafter\def\csname faicon@cc-mastercard\endcsname{{\FA\symbol{"F1F1}}}
\expandafter\def\csname faicon@cc-discover\endcsname{{\FA\symbol{"F1F2}}}
\expandafter\def\csname faicon@cc-amex\endcsname{{\FA\symbol{"F1F3}}}
\expandafter\def\csname faicon@cc-paypal\endcsname{{\FA\symbol{"F1F4}}}
\expandafter\def\csname faicon@cc-stripe\endcsname{{\FA\symbol{"F1F5}}}
\expandafter\def\csname faicon@bell-slash\endcsname{{\FA\symbol{"F1F6}}}
\expandafter\def\csname faicon@bell-slash-o\endcsname{{\FA\symbol{"F1F7}}}
\expandafter\def\csname faicon@trash\endcsname{{\FA\symbol{"F1F8}}}
\expandafter\def\csname faicon@copyright\endcsname{{\FA\symbol{"F1F9}}}
\expandafter\def\csname faicon@at\endcsname{{\FA\symbol{"F1FA}}}
\expandafter\def\csname faicon@eyedropper\endcsname{{\FA\symbol{"F1FB}}}
\expandafter\def\csname faicon@paint-brush\endcsname{{\FA\symbol{"F1FC}}}
\expandafter\def\csname faicon@birthday-cake\endcsname{{\FA\symbol{"F1FD}}}
\expandafter\def\csname faicon@area-chart\endcsname{{\FA\symbol{"F1FE}}}
\expandafter\def\csname faicon@pie-chart\endcsname{{\FA\symbol{"F200}}}
\expandafter\def\csname faicon@line-chart\endcsname{{\FA\symbol{"F201}}}
\expandafter\def\csname faicon@lastfm\endcsname{{\FA\symbol{"F202}}}
\expandafter\def\csname faicon@lastfm-square\endcsname{{\FA\symbol{"F203}}}
\expandafter\def\csname faicon@toggle-off\endcsname{{\FA\symbol{"F204}}}
\expandafter\def\csname faicon@toggle-on\endcsname{{\FA\symbol{"F205}}}
\expandafter\def\csname faicon@bicycle\endcsname{{\FA\symbol{"F206}}}
\expandafter\def\csname faicon@bus\endcsname{{\FA\symbol{"F207}}}
\expandafter\def\csname faicon@ioxhost\endcsname{{\FA\symbol{"F208}}}
\expandafter\def\csname faicon@angellist\endcsname{{\FA\symbol{"F209}}}
\expandafter\def\csname faicon@cc\endcsname{{\FA\symbol{"F20A}}}
\expandafter\def\csname faicon@ils\endcsname{{\FA\symbol{"F20B}}}
\expandafter\def\csname faicon@meanpath\endcsname{{\FA\symbol{"F20C}}}
\expandafter\def\csname faicon@buysellads\endcsname{{\FA\symbol{"F20D}}}
\expandafter\def\csname faicon@connectdevelop\endcsname{{\FA\symbol{"F20E}}}
\expandafter\def\csname faicon@dashcube\endcsname{{\FA\symbol{"F210}}}
\expandafter\def\csname faicon@forumbee\endcsname{{\FA\symbol{"F211}}}
\expandafter\def\csname faicon@leanpub\endcsname{{\FA\symbol{"F212}}}
\expandafter\def\csname faicon@sellsy\endcsname{{\FA\symbol{"F213}}}
\expandafter\def\csname faicon@shirtsinbulk\endcsname{{\FA\symbol{"F214}}}
\expandafter\def\csname faicon@simplybuilt\endcsname{{\FA\symbol{"F215}}}
\expandafter\def\csname faicon@skyatlas\endcsname{{\FA\symbol{"F216}}}
\expandafter\def\csname faicon@cart-plus\endcsname{{\FA\symbol{"F217}}}
\expandafter\def\csname faicon@cart-arrow-down\endcsname{{\FA\symbol{"F218}}}
\expandafter\def\csname faicon@diamond\endcsname{{\FA\symbol{"F219}}}
\expandafter\def\csname faicon@ship\endcsname{{\FA\symbol{"F21A}}}
\expandafter\def\csname faicon@user-secret\endcsname{{\FA\symbol{"F21B}}}
\expandafter\def\csname faicon@motorcycle\endcsname{{\FA\symbol{"F21C}}}
\expandafter\def\csname faicon@street-view\endcsname{{\FA\symbol{"F21D}}}
\expandafter\def\csname faicon@heartbeat\endcsname{{\FA\symbol{"F21E}}}
\expandafter\def\csname faicon@venus\endcsname{{\FA\symbol{"F221}}}
\expandafter\def\csname faicon@mars\endcsname{{\FA\symbol{"F222}}}
\expandafter\def\csname faicon@mercury\endcsname{{\FA\symbol{"F223}}}
\expandafter\def\csname faicon@transgender\endcsname{{\FA\symbol{"F224}}}
\expandafter\def\csname faicon@transgender-alt\endcsname{{\FA\symbol{"F225}}}
\expandafter\def\csname faicon@venus-double\endcsname{{\FA\symbol{"F226}}}
\expandafter\def\csname faicon@mars-double\endcsname{{\FA\symbol{"F227}}}
\expandafter\def\csname faicon@venus-mars\endcsname{{\FA\symbol{"F228}}}
\expandafter\def\csname faicon@mars-stroke\endcsname{{\FA\symbol{"F229}}}
\expandafter\def\csname faicon@mars-stroke-v\endcsname{{\FA\symbol{"F22A}}}
\expandafter\def\csname faicon@mars-stroke-h\endcsname{{\FA\symbol{"F22B}}}
\expandafter\def\csname faicon@neuter\endcsname{{\FA\symbol{"F22C}}}
\expandafter\def\csname faicon@genderless\endcsname{{\FA\symbol{"F22D}}}
\expandafter\def\csname faicon@facebook-official\endcsname{{\FA\symbol{"F230}}}
\expandafter\def\csname faicon@pinterest-p\endcsname{{\FA\symbol{"F231}}}
\expandafter\def\csname faicon@whatsapp\endcsname{{\FA\symbol{"F232}}}
\expandafter\def\csname faicon@server\endcsname{{\FA\symbol{"F233}}}
\expandafter\def\csname faicon@user-plus\endcsname{{\FA\symbol{"F234}}}
\expandafter\def\csname faicon@user-times\endcsname{{\FA\symbol{"F235}}}
\expandafter\def\csname faicon@bed\endcsname{{\FA\symbol{"F236}}}
\expandafter\def\csname faicon@viacoin\endcsname{{\FA\symbol{"F237}}}
\expandafter\def\csname faicon@train\endcsname{{\FA\symbol{"F238}}}
\expandafter\def\csname faicon@subway\endcsname{{\FA\symbol{"F239}}}
\expandafter\def\csname faicon@medium\endcsname{{\FA\symbol{"F23A}}}
\expandafter\def\csname faicon@y-combinator\endcsname{{\FA\symbol{"F23B}}}
\expandafter\def\csname faicon@optin-monster\endcsname{{\FA\symbol{"F23C}}}
\expandafter\def\csname faicon@opencart\endcsname{{\FA\symbol{"F23D}}}
\expandafter\def\csname faicon@expeditedssl\endcsname{{\FA\symbol{"F23E}}}
\expandafter\def\csname faicon@battery-full\endcsname{{\FA\symbol{"F240}}}
\expandafter\def\csname faicon@battery-three-quarters\endcsname{{\FA\symbol{"F241}}}
\expandafter\def\csname faicon@battery-half\endcsname{{\FA\symbol{"F242}}}
\expandafter\def\csname faicon@battery-quarter\endcsname{{\FA\symbol{"F243}}}
\expandafter\def\csname faicon@battery-empty\endcsname{{\FA\symbol{"F244}}}
\expandafter\def\csname faicon@mouse-pointer\endcsname{{\FA\symbol{"F245}}}
\expandafter\def\csname faicon@i-cursor\endcsname{{\FA\symbol{"F246}}}
\expandafter\def\csname faicon@object-group\endcsname{{\FA\symbol{"F247}}}
\expandafter\def\csname faicon@object-ungroup\endcsname{{\FA\symbol{"F248}}}
\expandafter\def\csname faicon@sticky-note\endcsname{{\FA\symbol{"F249}}}
\expandafter\def\csname faicon@sticky-note-o\endcsname{{\FA\symbol{"F24A}}}
\expandafter\def\csname faicon@cc-jcb\endcsname{{\FA\symbol{"F24B}}}
\expandafter\def\csname faicon@cc-diners-club\endcsname{{\FA\symbol{"F24C}}}
\expandafter\def\csname faicon@clone\endcsname{{\FA\symbol{"F24D}}}
\expandafter\def\csname faicon@balance-scale\endcsname{{\FA\symbol{"F24E}}}
\expandafter\def\csname faicon@hourglass-o\endcsname{{\FA\symbol{"F250}}}
\expandafter\def\csname faicon@hourglass-start\endcsname{{\FA\symbol{"F251}}}
\expandafter\def\csname faicon@hourglass-half\endcsname{{\FA\symbol{"F252}}}
\expandafter\def\csname faicon@hourglass-end\endcsname{{\FA\symbol{"F253}}}
\expandafter\def\csname faicon@hourglass\endcsname{{\FA\symbol{"F254}}}
\expandafter\def\csname faicon@hand-rock-o\endcsname{{\FA\symbol{"F255}}}
\expandafter\def\csname faicon@hand-paper-o\endcsname{{\FA\symbol{"F256}}}
\expandafter\def\csname faicon@hand-scissors-o\endcsname{{\FA\symbol{"F257}}}
\expandafter\def\csname faicon@hand-lizard-o\endcsname{{\FA\symbol{"F258}}}
\expandafter\def\csname faicon@hand-spock-o\endcsname{{\FA\symbol{"F259}}}
\expandafter\def\csname faicon@hand-pointer-o\endcsname{{\FA\symbol{"F25A}}}
\expandafter\def\csname faicon@hand-peace-o\endcsname{{\FA\symbol{"F25B}}}
\expandafter\def\csname faicon@trademark\endcsname{{\FA\symbol{"F25C}}}
\expandafter\def\csname faicon@registered\endcsname{{\FA\symbol{"F25D}}}
\expandafter\def\csname faicon@creative-commons\endcsname{{\FA\symbol{"F25E}}}
\expandafter\def\csname faicon@gg\endcsname{{\FA\symbol{"F260}}}
\expandafter\def\csname faicon@gg-circle\endcsname{{\FA\symbol{"F261}}}
\expandafter\def\csname faicon@tripadvisor\endcsname{{\FA\symbol{"F262}}}
\expandafter\def\csname faicon@odnoklassniki\endcsname{{\FA\symbol{"F263}}}
\expandafter\def\csname faicon@odnoklassniki-square\endcsname{{\FA\symbol{"F264}}}
\expandafter\def\csname faicon@get-pocket\endcsname{{\FA\symbol{"F265}}}
\expandafter\def\csname faicon@wikipedia-w\endcsname{{\FA\symbol{"F266}}}
\expandafter\def\csname faicon@safari\endcsname{{\FA\symbol{"F267}}}
\expandafter\def\csname faicon@chrome\endcsname{{\FA\symbol{"F268}}}
\expandafter\def\csname faicon@firefox\endcsname{{\FA\symbol{"F269}}}
\expandafter\def\csname faicon@opera\endcsname{{\FA\symbol{"F26A}}}
\expandafter\def\csname faicon@internet-explorer\endcsname{{\FA\symbol{"F26B}}}
\expandafter\def\csname faicon@television\endcsname{{\FA\symbol{"F26C}}}
\expandafter\def\csname faicon@contao\endcsname{{\FA\symbol{"F26D}}}
\expandafter\def\csname faicon@500px\endcsname{{\FA\symbol{"F26E}}}
\expandafter\def\csname faicon@amazon\endcsname{{\FA\symbol{"F270}}}
\expandafter\def\csname faicon@calendar-plus-o\endcsname{{\FA\symbol{"F271}}}
\expandafter\def\csname faicon@calendar-minus-o\endcsname{{\FA\symbol{"F272}}}
\expandafter\def\csname faicon@calendar-times-o\endcsname{{\FA\symbol{"F273}}}
\expandafter\def\csname faicon@calendar-check-o\endcsname{{\FA\symbol{"F274}}}
\expandafter\def\csname faicon@industry\endcsname{{\FA\symbol{"F275}}}
\expandafter\def\csname faicon@map-pin\endcsname{{\FA\symbol{"F276}}}
\expandafter\def\csname faicon@map-signs\endcsname{{\FA\symbol{"F277}}}
\expandafter\def\csname faicon@map-o\endcsname{{\FA\symbol{"F278}}}
\expandafter\def\csname faicon@map\endcsname{{\FA\symbol{"F279}}}
\expandafter\def\csname faicon@commenting\endcsname{{\FA\symbol{"F27A}}}
\expandafter\def\csname faicon@commenting-o\endcsname{{\FA\symbol{"F27B}}}
\expandafter\def\csname faicon@houzz\endcsname{{\FA\symbol{"F27C}}}
\expandafter\def\csname faicon@vimeo\endcsname{{\FA\symbol{"F27D}}}
\expandafter\def\csname faicon@black-tie\endcsname{{\FA\symbol{"F27E}}}
\expandafter\def\csname faicon@fonticons\endcsname{{\FA\symbol{"F280}}}
\expandafter\def\csname faicon@reddit-alien\endcsname{{\FA\symbol{"F281}}}
\expandafter\def\csname faicon@edge\endcsname{{\FA\symbol{"F282}}}
\expandafter\def\csname faicon@credit-card-alt\endcsname{{\FA\symbol{"F283}}}
\expandafter\def\csname faicon@codiepie\endcsname{{\FA\symbol{"F284}}}
\expandafter\def\csname faicon@modx\endcsname{{\FA\symbol{"F285}}}
\expandafter\def\csname faicon@fort-awesome\endcsname{{\FA\symbol{"F286}}}
\expandafter\def\csname faicon@usb\endcsname{{\FA\symbol{"F287}}}
\expandafter\def\csname faicon@product-hunt\endcsname{{\FA\symbol{"F288}}}
\expandafter\def\csname faicon@mixcloud\endcsname{{\FA\symbol{"F289}}}
\expandafter\def\csname faicon@scribd\endcsname{{\FA\symbol{"F28A}}}
\expandafter\def\csname faicon@pause-circle\endcsname{{\FA\symbol{"F28B}}}
\expandafter\def\csname faicon@pause-circle-o\endcsname{{\FA\symbol{"F28C}}}
\expandafter\def\csname faicon@stop-circle\endcsname{{\FA\symbol{"F28D}}}
\expandafter\def\csname faicon@stop-circle-o\endcsname{{\FA\symbol{"F28E}}}
\expandafter\def\csname faicon@shopping-bag\endcsname{{\FA\symbol{"F290}}}
\expandafter\def\csname faicon@shopping-basket\endcsname{{\FA\symbol{"F291}}}
\expandafter\def\csname faicon@hashtag\endcsname{{\FA\symbol{"F292}}}
\expandafter\def\csname faicon@bluetooth\endcsname{{\FA\symbol{"F293}}}
\expandafter\def\csname faicon@bluetooth-b\endcsname{{\FA\symbol{"F294}}}
\expandafter\def\csname faicon@percent\endcsname{{\FA\symbol{"F295}}}
\expandafter\def\csname faicon@gitlab\endcsname{{\FA\symbol{"F296}}}
\expandafter\def\csname faicon@wpbeginner\endcsname{{\FA\symbol{"F297}}}
\expandafter\def\csname faicon@wpforms\endcsname{{\FA\symbol{"F298}}}
\expandafter\def\csname faicon@envira\endcsname{{\FA\symbol{"F299}}}
\expandafter\def\csname faicon@universal-access\endcsname{{\FA\symbol{"F29A}}}
\expandafter\def\csname faicon@wheelchair-alt\endcsname{{\FA\symbol{"F29B}}}
\expandafter\def\csname faicon@question-circle-o\endcsname{{\FA\symbol{"F29C}}}
\expandafter\def\csname faicon@blind\endcsname{{\FA\symbol{"F29D}}}
\expandafter\def\csname faicon@audio-description\endcsname{{\FA\symbol{"F29E}}}
\expandafter\def\csname faicon@volume-control-phone\endcsname{{\FA\symbol{"F2A0}}}
\expandafter\def\csname faicon@braille\endcsname{{\FA\symbol{"F2A1}}}
\expandafter\def\csname faicon@assistive-listening-systems\endcsname{{\FA\symbol{"F2A2}}}
\expandafter\def\csname faicon@american-sign-language-interpreting\endcsname{{\FA\symbol{"F2A3}}}
\expandafter\def\csname faicon@deaf\endcsname{{\FA\symbol{"F2A4}}}
\expandafter\def\csname faicon@glide\endcsname{{\FA\symbol{"F2A5}}}
\expandafter\def\csname faicon@glide-g\endcsname{{\FA\symbol{"F2A6}}}
\expandafter\def\csname faicon@sign-language\endcsname{{\FA\symbol{"F2A7}}}
\expandafter\def\csname faicon@low-vision\endcsname{{\FA\symbol{"F2A8}}}
\expandafter\def\csname faicon@viadeo\endcsname{{\FA\symbol{"F2A9}}}
\expandafter\def\csname faicon@viadeo-square\endcsname{{\FA\symbol{"F2AA}}}
\expandafter\def\csname faicon@snapchat\endcsname{{\FA\symbol{"F2AB}}}
\expandafter\def\csname faicon@snapchat-ghost\endcsname{{\FA\symbol{"F2AC}}}
\expandafter\def\csname faicon@snapchat-square\endcsname{{\FA\symbol{"F2AD}}}
\expandafter\def\csname faicon@pied-piper\endcsname{{\FA\symbol{"F2AE}}}
\expandafter\def\csname faicon@first-order\endcsname{{\FA\symbol{"F2B0}}}
\expandafter\def\csname faicon@yoast\endcsname{{\FA\symbol{"F2B1}}}
\expandafter\def\csname faicon@themeisle\endcsname{{\FA\symbol{"F2B2}}}
\expandafter\def\csname faicon@google-plus-official\endcsname{{\FA\symbol{"F2B3}}}
\expandafter\def\csname faicon@font-awesome\endcsname{{\FA\symbol{"F2B4}}}


==> implem.tex <==
% \subsection{Tool Implementation}
We have implemented {\sc SmartEmbed} as a standalone web service to facilitate Solidity developers in checking their smart contracts. The source code and data can be found in our Github repository\footnote{\url{https://github.com/beyondacm/SmartEmbed}}.

\smallskip
\noindent{\itshape\bfseries Data Collection}.
%\subsection{Data Collection}
We collected 22,275 verified Solidity smart contracts using EtherScan\footnote{https://etherscan.io/}, which is a block explorer and analytics platform for Ethereum.
%By the time of our data collection, there were 22,725 verified contracts on Etherscan, 
The contracts contain 135,239 subcontracts, 631,261 functions, around 2 million statements, and more than 7 million lines of code.
In the meanwhile, we collected 22 well-known vulnerable smart contracts and pinpointed 37 buggy statements in the contracts, which served as the bug database for {\sc SmartEmbed}.

\smallskip
\noindent{\itshape\bfseries Backend Model}.
%\subsection{Backend Model}
The collected source code of contracts are inputted into the workflow of our approach described in Section ~\ref{sec:approach}, and the output is the code embeddings which are used by {\sc SmartEmbed} as the backend model for similarity checking.

\smallskip
\noindent{\itshape\bfseries Frontend User Interface}.
%\subsection{Frontend User Interface}
On the user interface, {\sc SmartEmbed} provides an input box for Solidity developers to submit their source code (cf.\ Fig.~\ref{fig:tool-clone} and Fig.~\ref{fig:tool-bug}). 
After a Solidity developer submits his/her source code to the server, the source code is parsed and normalized, then the contract and each statement is converted into a vector by our code embedding model for similarity checking.
The outputs are organised into two separate result tabs for clone detection and bug detection respectively.
For the clone detection result tab, {\sc SmartEmbed} returns top-5 most similar clone contracts in our code base together with the similarity scores and links to their locations in EtherScan (cf.\ Fig.~\ref{fig:tool-clone}).
For the bug detection result tab, the {\sc SmartEmbed} highlights the buggy lines in the submitted source code and reports the bug types back to the developer (cf.\ Fig.~\ref{fig:tool-bug}).
%Fig.~\ref{fig:tool-clone} and Fig.~\ref{fig:tool-bug} shows the results of clone detection and bug detection by our tool. 

\begin{figure}[t]
    \centerline{\includegraphics[width=0.43\textwidth]{tool-clone-detection-print.pdf}}
\vspace*{-10pt}
\caption{Sample Results of Clone Detection}\vspace*{-0.4cm}
\label{fig:tool-clone}
\end{figure}


\begin{figure}[t]
    \centerline{\includegraphics[width=0.43\textwidth]{tool-bug-detection-print.pdf}}
\vspace*{-10pt}
\caption{Sample Results of Bug Detection}\vspace*{-0.6cm}
\label{fig:tool-bug}
\end{figure}
